A basic time series forecasting course with Python

The aim of this paper is to present a set of Python-based tools to develop forecasts using time series data sets. The material is based on a four week course that the author has taught for seven years to students on operations research, management science, analytics, and statistics one-year MSc programmes. However, it can easily be adapted to various other audiences, including executive management or some undergraduate programmes. No particular knowledge of Python is required to use this material. Nevertheless, we assume a good level of familiarity with standard statistical forecasting methods such as exponential smoothing, AutoRegressive Integrated Moving Average (ARIMA), and regression-based techniques, which is required to deliver such a course. Access to relevant data, codes, and lecture notes, which serve as based for this material are made available (see github.com/abzemkoho/forecasting) for anyone interested in teaching such a course or developing some familiarity with the mathematical background of relevant methods and tools.

==> Source file of paper - final/appendices.tex <==
\appendix

\section{Codes on preliminaries on python and data analysis}


\begin{lstlisting}[language=Python, caption={TimePlot}, label={TimePlot}]
from pandas import read_excel
from matplotlib import pyplot
series = read_excel('ClayBricks.xls', sheetname='BRICKSQ', header=0,
              index_col=0, parse_dates=True, squeeze=True)
series.plot()
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={SeasonalPlot}, label={SeasonalPlot}]
from pandas import read_excel
import matplotlib.pyplot as plt
import numpy as np
series = read_excel('ClayBricks.xls',
              sheetname='SeasonalData', header=0, index_col=0, parse_dates=True, squeeze=True)
x = np.array([0,1,2,3,4,5,6,7,8,9,10,11])
months = ['Jan','Feb','Mar','Apr', 'May', 'Jun', 'Jul', 'Aug', 'Sep', 'Oct', 'Nov', 'Dec']
plt.xticks(x, months)
plt.plot(x, series)
plt.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={LogTransform}, label={LogTransform}]
from pandas import read_excel
from pandas import DataFrame
from numpy import log
from matplotlib import pyplot
series = read_excel('Electricity.xls',
              sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
dataframe = DataFrame(series.values)
dataframe.columns = ['electricity']
dataframe['electricity'] = log(dataframe['electricity'])
pyplot.figure(1)
# line plot
pyplot.subplot(211)
pyplot.plot(dataframe['electricity'])
# histogram
pyplot.subplot(212)
pyplot.hist(dataframe['electricity'])
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={SqrtTransform}, label={SqrtTransform}]
from pandas import read_excel
from pandas import DataFrame
from numpy import sqrt
from matplotlib import pyplot
series = read_excel('Electricity.xls',
              sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
dataframe = DataFrame(series.values)
dataframe.columns = ['electricity']
dataframe['electricity'] = sqrt(dataframe['electricity'])
pyplot.figure(1)
# line plot
pyplot.subplot(211)
pyplot.plot(dataframe['electricity'])
# histogram
pyplot.subplot(212)
pyplot.hist(dataframe['electricity'])
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={CalendarAdjustment}, label={CalendarAdjustment}]
from pandas import read_excel
from matplotlib import pyplot
series = read_excel('MilkProduction.xls',
              sheetname='AdjustedData', header=0,
              index_col=0, parse_dates=True, squeeze=True)  # you can include various other parameters
series.plot()
pyplot.show()
\end{lstlisting}




%\begin{lstlisting}[language=Python, caption=Demo 1.3 (code plotting the scatter plot for the used cars vs their current milleage)]
%import pandas as pd
%import matplotlib.pyplot as plt
%#import numpy as np
%from pandas import read_excel
%series1 = read_excel('JapaneseCars.xls', sheet_name='Data', usecols = [0], header=0,
%                     squeeze=True, dtype=float)
%series2 = read_excel('JapaneseCars.xls', sheet_name='Data', usecols=[1], header=0,
%                     squeeze=True, dtype=float)
%
%Japanese = {'Mileage': series1, 'Price': series2}
%df = pd.DataFrame(Japanese, columns=['Mileage', 'Price'])
%plt.scatter(df.Mileage, df.Price)
%
%plt.xlabel('Mileage (MPG)')
%plt.ylabel('Price (US$)')
%plt.title('Price/Mileage Relationship for 19 Japanese cars')
%\end{lstlisting}


\begin{lstlisting}[language=Python,  caption={Correlation}, label={correlation}]
from pandas import read_excel
import numpy as np
series1 = read_excel('JapaneseCars.xls', sheet_name='Data', usecols = [0], header=0,
                     squeeze=True, dtype=float)
series2 = read_excel('JapaneseCars.xls', sheet_name='Data', usecols=[1], header=0,
                     squeeze=True, dtype=float)
correlval=np.corrcoef(series1, series2)
correlval=correlval[1,0]
print(correlval)
\end{lstlisting}

%\begin{lstlisting}[language=Python, caption=Demo 1.5 (Calculating/plotting/representing the autocorrelation), label={autocorrelation1}]
%# create an autocorrelation plot
%from pandas import read_excel
%from matplotlib import pyplot
%from pandas.plotting import autocorrelation_plot
%series = read_excel('Beer.xls', sheet_name='Data', header=0, index_col=0, parse_dates=True, squeeze=True)
%autocorrelation_plot(series)
%pyplot.show()
%\end{lstlisting}
%
%
%\begin{lstlisting}[language=Python, caption=Demo 1.6 (Trend estimation/calculation/representation)]
%from pandas import read_excel
%from matplotlib import pyplot
%series = read_excel('HouseSales.xls',
%              sheetname='MAData', header=0,
%              index_col=0, parse_dates=True, squeeze=True)  # you can include various other parameters
%series.plot()
%pyplot.show()
%\end{lstlisting}
%
\begin{lstlisting}[language=Python, caption={DecompositionAdditive}, label={DecompositionAdditive}]
from pandas import read_excel
from matplotlib import pyplot
from statsmodels.tsa.seasonal import seasonal_decompose
series = read_excel('HouseSales.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
result = seasonal_decompose(series, model='additive')
#result = seasonal_decompose(series, model='multiplicative')
result.plot()
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={DecompositionMultiplicative}, label={DecompositionMultiplicative}]
from pandas import read_excel
from matplotlib import pyplot
from statsmodels.tsa.seasonal import seasonal_decompose
series = read_excel('AirlineSales.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
#result = seasonal_decompose(series, model='additive')
result = seasonal_decompose(series, model='multiplicative')
result.plot()
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={CorrelationMatrix}, label={CorrelationMatrix}]
from pandas import read_excel
import matplotlib.pyplot as plt
import pandas as pd
series = read_excel('Bank.xls', sheet_name='Data3', header=0,
                     squeeze=True, dtype=float)

#Plotting the scatter plots of each variable against the other one
pd.plotting.scatter_matrix(series, figsize=(8, 8))
plt.show()

# Correlation matrix for all the variables, 2 by 2
CorrelationMatrix = series.corr()
print(CorrelationMatrix)
# As in the case of Demo 1.4, corrcoef can be used for the variables in couples.
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={Autocorrelation}, label={Autocorrelation}]
from pandas import read_excel
from matplotlib import pyplot
from pandas.plotting import autocorrelation_plot
from statsmodels.graphics.tsaplots import plot_acf
series1 = read_excel('CementProduction.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
series2 = read_excel('CementProduction.xls', sheetname='SeasonalData', header=0,
                    index_col=0, parse_dates=True, squeeze=True)
series2.plot(title='Seasonal plots building materials time series')
pyplot.show()

plot_acf(series1, title='ACF plot of building materials time series', lags=60)
pyplot.show()

autocorrelation_plot(series1)
pyplot.show()
\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Codes on exponential smoothing methods}

\begin{lstlisting}[language=Python, caption={ErrorMeasures}, label={ErrorMeasures}]
from pandas import read_excel
from matplotlib import pyplot
AustralianBeer  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [1],
                             header=0, squeeze=True, dtype=float)
NaiveF1  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [2],
                      header=0, squeeze=True, dtype=float)
NaiveF2 = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols=[3],
                     header=0, squeeze=True, dtype=float)

# Joint plot of original data and NF1 forecasts
AustralianBeer.plot(legend=True)
NaiveF1.plot(legend=True)
pyplot.show()

# Joint plot of original data and NF2 forecasts
AustralianBeer.plot(legend=True)
NaiveF2.plot(legend=True)
pyplot.show()

# Evaluating the errors from both NF1 and NF2 methods
Error1 = AustralianBeer - NaiveF1
Error2 = AustralianBeer - NaiveF2
ME1 = sum(Error1)* 1.0/len(NaiveF1)
ME2 = sum(Error2)* 1.0/len(NaiveF2)
MAE1=sum(abs(Error1))*1.0/len(NaiveF1)
MAE2=sum(abs(Error2))*1.0/len(NaiveF2)
MSE1=sum(Error1**2)*1.0/len(NaiveF1)
MSE2=sum(Error2**2)*1.0/len(NaiveF2)

PercentageError1=(Error1/AustralianBeer)*100
PercentageError2=(Error2/AustralianBeer)*100
MPE1 = sum(PercentageError1)* 1.0/len(NaiveF1)
MPE2 = sum(PercentageError2)* 1.0/len(NaiveF2)
MAE1=sum(abs(PercentageError1))*1.0/len(NaiveF1)
MAE2=sum(abs(PercentageError2))*1.0/len(NaiveF2)


#Printing a summary of the errors in a tabular form
print('Summary of errors resulting from NF1 & NF2:')
import pandas as pd
cars = {'Errors': ['ME','MAE','MSE','MPE', 'MAPE'],
        'NF1': [ME1, MAE1, MSE1, MPE1, MAE1],
        'NF2': [ME2, MAE2, MSE2, MPE2, MAE2]
        }
AllErrors = pd.DataFrame(cars, columns = ['Errors', 'NF1', 'NF2'])
print(AllErrors)
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={ACFErrors}, label={ACFErrors}]
from pandas import read_excel
from matplotlib import pyplot
AustralianBeer  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [1],
                             header=0, squeeze=True, dtype=float)
NaiveF1  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [2],
                      header=0, squeeze=True, dtype=float)
NaiveF2 = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols=[3],
                     header=0, squeeze=True, dtype=float)

# Plot for the original data set
AustralianBeer.plot(label='Original data', legend=True)
pyplot.show()

# Evaluating the errors from both NF1 and NF2 methods
Error1 = AustralianBeer - NaiveF1
Error2 = AustralianBeer - NaiveF2

# Plot of the error time series
Error1.plot(label='NF1 error plot', legend=True)
Error2.plot(label='NF2 error plot', legend=True)
pyplot.show()

# Creating an autocorrelation plot
from pandas.plotting import autocorrelation_plot
autocorrelation_plot(Error1)
autocorrelation_plot(Error2)
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={ConfidenceInterval}, label={ConfidenceInterval}]
from pandas import read_excel
from matplotlib import pyplot
from numpy import sqrt
AustralianBeer  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [1],
                             header=0, squeeze=True, dtype=float)
NaiveF1  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [2],
                      header=0, squeeze=True, dtype=float)
NaiveF2 = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols=[3],
                     header=0, squeeze=True, dtype=float)



# Evaluating the errors from both NF1 and NF2 methods
Error1 = AustralianBeer - NaiveF1
Error2 = AustralianBeer - NaiveF2
MSE1=sum(Error1**2)*1.0/len(NaiveF1)
MSE2=sum(Error2**2)*1.0/len(NaiveF2)

LowerForecast1 = NaiveF1 - 1.645*sqrt(MSE1)
UpperForecast1 = NaiveF1 + 1.645*sqrt(MSE1)

LowerForecast2 = NaiveF2 - 1.645*sqrt(MSE2)
UpperForecast2 = NaiveF2 + 1.645*sqrt(MSE2)

# Joint plot of original data and NF1 forecasts
AustralianBeer.plot(label='Original data')
NaiveF1.plot(label='NF1 forecast')
LowerForecast1.plot(label='NF1 lower bound')
UpperForecast1.plot(label='NF1 upper bound')
pyplot.legend()
pyplot.show()

# Joint plot of original data and NF2 forecasts
AustralianBeer.plot(label='Original data')
NaiveF2.plot(label='NF2 forecast')
LowerForecast2.plot(label='NF2 lower bound')
UpperForecast2.plot(label='NF2 upper bound')
pyplot.legend()
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={SimpleExpSmoothing}, label={SimpleExpSmoothing}]
from pandas import read_excel
from statsmodels.tsa.api import SimpleExpSmoothing
from matplotlib import pyplot
series = read_excel('ShampooSales.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)

# Simple Exponential Smoothing #

## SES model 1: alpha = 0.1
fit1 = SimpleExpSmoothing(series).fit(smoothing_level=0.1,optimized=False)
fcast1 = fit1.forecast(10).rename(r'$\alpha=0.1$')
# Plot of fitted values and forecast of next 10 values, respectively
fit1.fittedvalues.plot(color='blue')
fcast1.plot(color='blue', legend=True)

## SES model 2: alpha = 0.7
fit2 = SimpleExpSmoothing(series).fit(smoothing_level=0.7,optimized=False)
fcast2 = fit2.forecast(10).rename(r'$\alpha=0.7$')
# Plot of fitted values and forecast of next 10 values, respectively
fcast2.plot(color='red', legend=True)
fit2.fittedvalues.plot(color='red')

## SES model 3: alpha automatically selected by the built-in optimization software
fit3 = SimpleExpSmoothing(series).fit()
fcast3 = fit3.forecast(10).rename(r'$\alpha=%s$'%fit3.model.params['smoothing_level'])
# Plot of fitted values and forecast of next 10 values, respectively
fcast3.plot(color='green', legend=True)
fit3.fittedvalues.plot(color='green')

# Plotting the original data together with the 3 forecast plots
series.plot(color='black', legend=True)
pyplot.show()

#Evaluating the errors
from sklearn.metrics import mean_squared_error
MSE1=mean_squared_error(fit1.fittedvalues, series)
MSE2=mean_squared_error(fit2.fittedvalues, series)
MSE3=mean_squared_error(fit3.fittedvalues, series)

print('Summary of errors resulting from SES models 1, 2 & 3:')
import pandas as pd
cars = {'Model': ['MSE'],
        'SES model 1': [MSE1],
        'SES model 2': [MSE2],
        'SES model 3': [MSE3]
        }
AllErrors = pd.DataFrame(cars, columns = ['Model', 'SES model 1', 'SES model 2', 'SES model 3'])
print(AllErrors)
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={Holt}, label={Holt}]
from pandas import read_excel
from statsmodels.tsa.api import Holt
from matplotlib import pyplot
series = read_excel('ShampooSales.xls', sheetname='Data', header=0,
              index_col=0, squeeze=True)

# Holt model 1: alpha = 0.8, beta=0.2
fit1 = Holt(series).fit(smoothing_level=0.8, smoothing_slope=0.2, optimized=False)
fcast1 = fit1.forecast(12).rename("Holt's linear trend")

fit2 = Holt(series, exponential=True).fit(smoothing_level=0.8, smoothing_slope=0.2, optimized=False)
fcast2 = fit2.forecast(12).rename("Exponential trend")

fit3 = Holt(series, damped=True).fit(smoothing_level=0.8, smoothing_slope=0.2)
fcast3 = fit3.forecast(12).rename("Additive damped trend")

fit4 = Holt(series).fit(optimized=True)
fcast4 = fit4.forecast(12).rename("Additive 2 damped trend")


fit1.fittedvalues.plot(color='blue')
fcast1.plot(color='blue', legend=True)

fit2.fittedvalues.plot(color='red')
fcast2.plot(color='red', legend=True)

fit3.fittedvalues.plot(color='green')
fcast3.plot(color='green', legend=True)

fcast4.plot(color='yellow', legend=True)

series.plot(color='black', legend=True)
pyplot.show()

#Evaluating the errors
from sklearn.metrics import mean_squared_error
MSE1=mean_squared_error(fit1.fittedvalues, series)
MSE2=mean_squared_error(fit2.fittedvalues, series)
MSE3=mean_squared_error(fit3.fittedvalues, series)

print('Summary of errors resulting from SES models 1, 2 & 3:')
import pandas as pd
cars = {'Model': ['MSE'],
        'LES model 1': [MSE1],
        'LES model 2': [MSE2],
        'LES model 3': [MSE3]
        }
AllErrors = pd.DataFrame(cars, columns = ['Model', 'LES model 1', 'LES model 2', 'LES model 3'])
print(AllErrors)
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={ExponentialSmoothing}, label={ExponentialSmoothing}]
from pandas import read_excel
import pandas as pd
from statsmodels.tsa.api import ExponentialSmoothing
from matplotlib import pyplot
series = read_excel('CementProduction.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)

# ===================================
# Holt-Winter method in different scenarios #
# ===================================
# ===================================
# Model 1: Holt-Winter method with additive trend and seasonality
# Here, alpha = 0.3, beta=0.5, gamma=0.7
# ===================================
fit1 = ExponentialSmoothing(series, seasonal_periods=12, trend='add', seasonal='add').fit(smoothing_level = 0.3, smoothing_slope=0.5,  smoothing_seasonal=0.7)
fit1.fittedvalues.plot(color='red')

# ===================================
# Model 2: Holt-Winter method with additive trend and multiplicative seasonality
# Here, alpha = 0.3, beta=0.5, gamma=0.7
# ===================================
fit2 = ExponentialSmoothing(series, seasonal_periods=12, trend='add', seasonal='mul').fit(smoothing_level = 0.3, smoothing_slope=0.5,  smoothing_seasonal=0.7)
fit2.fittedvalues.plot(color='blue')

# ===================================
# Model 3: Holt-Winter method with additive trend and seasonality
# Here, the parameters alpha, beta, and gamma are optimized
# ===================================
fit3 = ExponentialSmoothing(series, seasonal_periods=12, trend='add', seasonal='add').fit()
fit3.fittedvalues.plot(color='green')

# ===================================
# Model 4: Holt-Winter method with additive trend and multiplicative seasonality
# Here, the parameters alpha, beta, and gamma are optimized
# ===================================
fit4 = ExponentialSmoothing(series, seasonal_periods=12, trend='add', seasonal='mul').fit()
fit4.fittedvalues.plot(color='yellow')

print("Forecasting Cement Production with Holt-Winters method")
#=====================================
# Time and forecast plots
#=====================================
series.rename('Time plot of original series').plot(color='black', legend=True)
fit1.forecast(12).rename('Model 1: HW-additive seasonality').plot(color='red', legend=True)
fit2.forecast(12).rename('Model 2: HW-multiplicative seasonality').plot(color='blue', legend=True)
fit3.forecast(12).rename('Model 3: Opt HW-additive seasonality').plot(color='green', legend=True)
fit4.forecast(12).rename('Model 4: Opt HW-multiplicative seasonality').plot(color='yellow', legend=True)
pyplot.xlabel('Dates')
pyplot.ylabel('Values')
pyplot.title('HW method-based forecasts for cement production')
pyplot.show()


#====================================
# Evaluating the errors
#====================================
from sklearn.metrics import mean_squared_error
MSE1=mean_squared_error(fit1.fittedvalues, series)
MSE2=mean_squared_error(fit2.fittedvalues, series)
MSE3=mean_squared_error(fit3.fittedvalues, series)
MSE4=mean_squared_error(fit4.fittedvalues, series)

#=====================================
# Printing the paramters and errors for each scenario
#=====================================
results=pd.DataFrame(index=[r"alpha", r"beta", r"gamma", r"l0", "b0", "MSE"])
params = ['smoothing_level', 'smoothing_slope', 'smoothing_seasonal', 'initial_level', 'initial_slope']
results["HW model 1"] = [fit1.params[p] for p in params] + [MSE1]
results["HW model 2"] = [fit2.params[p] for p in params] + [MSE2]
results["HW model 3"] = [fit3.params[p] for p in params] + [MSE3]
results["HW model 4"] = [fit4.params[p] for p in params] + [MSE4]
print(results)

#=====================================
# Evaluating and plotting the residual series for each scenario
#=====================================
residuals1= fit1.fittedvalues - series
residuals2= fit2.fittedvalues - series
residuals3= fit3.fittedvalues - series
residuals4= fit4.fittedvalues - series
residuals1.rename('residual plot for model 1').plot(color='red', legend=True)
residuals2.rename('residual plot for model 2').plot(color='blue', legend=True)
residuals3.rename('residual plot for model 3').plot(color='green', legend=True)
residuals4.rename('residual plot for model 4').plot(color='yellow', legend=True)
pyplot.title('Residual plots for models 1-4')
pyplot.show()

#=====================================
# ACF plots of the residual series for each scenario
#=====================================
from statsmodels.graphics.tsaplots import plot_acf
plot_acf(residuals1, title='Residual ACF for model 1', lags=50)
plot_acf(residuals2, title='Residual ACF for model 2', lags=50)
plot_acf(residuals3, title='Residual ACF for model 3', lags=50)
plot_acf(residuals4, title='Residual ACF for model 4', lags=50)
pyplot.show()
\end{lstlisting}

\section{Codes on ARIMA methods}
\begin{lstlisting}[language=Python, caption={WhiteNoiseModel}, label={WhiteNoiseModel}]
from random import gauss
from random import seed
from pandas import Series
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
from matplotlib import pyplot

# seed random number generator
seed(1)
# create white noise series
series = [gauss(0.0, 1.0) for i in range(1000)]

# Once created, we can wrap the list in a Pandas Series for convenience.
series = Series(series)

# summary statistics of the artificially generated series
print('Statistics of the artificially generated series:')
print(series.describe())

# line plot of the artificially generated series
series.plot(title='Time plot of a white noise model')
pyplot.show()

# histogram plot of the artificially generated series
series.hist()

# ACF plot of an artificially generated white noise time series
plot_acf(series, title='ACF of a white noise model', lags=50)

# PACF plot of an artificially generated white noise time series
plot_pacf(series, title='PACF of a white noise model', lags=50)
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={AcfPacfPlotNonStationarity.py}, label={AcfPacfPlotDowJones.py}]
from pandas import read_excel
from matplotlib import pyplot
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
series = read_excel('DowJones.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)

# ACF plot on 50 time lags
plot_acf(series, title='ACF of Dow Jones time series', lags=50)

# PACF plot on 50 time lags
plot_pacf(series, title='PACF of Dow Jones time series', lags=50)
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={ADFtest.py}, label={ADFtest.py}]
from pandas import read_excel
import matplotlib.pyplot as plt
series = read_excel('BuildingMaterials.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
series.plot(color='red')
plt.xlabel('Dates')
plt.ylabel('Production values')
plt.title('Building materials production from 1986 to 2008')
plt.show()
#------------------------
from pandas import read_excel
from matplotlib import pyplot
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
series = read_excel('BuildingMaterials.xls', sheet_name='Data', usecols = [1],
                             header=0, squeeze=True, dtype=float)
# ACF plot on 50 time lags
plot_acf(series, title='ACF of building materials time series', lags=50)

# PACF plot on 50 time lags
plot_pacf(series, title='PACF of building materials time series', lags=50)
pyplot.show()
#--------------------------------------------------
# calculate stationarity test of time series data
#from pandas import read_csv
from statsmodels.tsa.stattools import adfuller
#series = read_csv('airline-passengers.csv', header=0, index_col=0, parse_dates=True,squeeze=True)
X = series.values
result = adfuller(X)
print('ADF Statistic: %f' % result[0])
print('p-value: %f' % result[1])
print('Critical Values:')
for key, value in result[4].items():
    print('\t%s: %.3f' % (key, value))
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={AcfPacfAR1model.py}, label={AcfPacfAR1model.py}]
from pandas import read_excel
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
from matplotlib import pyplot

series = read_excel('DataAR1model.xls', sheet_name='ARdata', header=0, index_col=0, squeeze=True)

# Time, ACF, and PACF plots for original data
pyplot.plot(series)
pyplot.title('Time plot AR1 data')
plot_acf(series, title='ACF plot of AR1 data', lags=20)
plot_pacf(series, title='PACF plot of AR1 data', lags=20)
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={AcfPacfMA1model.py}, label={AcfPacfMA1model.py}]
from pandas import read_excel
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
from matplotlib import pyplot

series = read_excel('DataMA1model.xls', sheet_name='MAdata', usecols = [1],
                    header=0, squeeze=True)

# Time, ACF, and PACF plots for original data
pyplot.plot(series)
pyplot.title('Time plot MA1 data')
plot_acf(series, title='ACF plot of MA1 data', lags=20)
plot_pacf(series, title='PACF plot of MA1 data', lags=20)
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={AutomaticOrderARIMA.py}, label={AutomaticOrderARIMA.py}]
#===================================================
#Code for identifying the parameters with smallest AIC
#===================================================
from pandas import read_excel
from statsmodels.tsa.arima_model import ARIMA
import warnings
import itertools

series = read_excel('BuildingMaterials.xls', sheet_name='Data', header=0, index_col=0, parse_dates=True, squeeze=True)

#define the p, d and q parameters to take any value between 0 and 2
p = d = q = range(0, 3)

#generate all different combinations of p, q and q triplets
pdq = list(itertools.product(p, d, q))

#indentification of best model from different combinations of pdq
warnings.filterwarnings("ignore") # specify to ignore warning messages
best_score, best_param = float("inf"), None
for param in pdq:
        try:
            mod = ARIMA(series, param)
            results = mod.fit()
            if results.aic < best_score:
                best_score, best_param = results.aic, param
            print('ARIMA{} - AIC:{}'.format(param, results.aic))
        except:
            continue
print('The best model is ARIMA{} - AIC:{}'.format(best_param, best_score))
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={ARIMA.py}, label={ARIMA.py}]
from pandas import read_excel
import matplotlib.pyplot as plt
from statsmodels.tsa.arima_model import ARIMA

series = read_excel('BuildingMaterials.xls', sheet_name='Data', header=0,
                index_col=0, parse_dates=True, squeeze=True)

#ARIMA(1,1,2) model
model = ARIMA(series, order=(1,1,2))

# generates ARIMA Model Results table
model_fit = model.fit(disp=0)
fitted = model.fit(disp=1)
print(model_fit.summary())

# Actual vs Fitted
model_fit.plot_predict(dynamic=False)
plt.show()

# Forecast
fc, se, conf = fitted.forecast(15, alpha=0.005)  # 95% conf

pred_ci = pred_uc.conf_int()
# plotting forecasts ahead
ax = series.plot(label='Original data')
pred_uc.predicted_mean.plot(ax=ax, label='Forecast values', title='Forecast plot with confidence interval')
ax.fill_between(pred_ci.index,
                pred_ci.iloc[:, 0],
                pred_ci.iloc[:, 1], color='k', alpha=.25)
plt.legend()
plt.show()
#====================================================================

#====================================================================
# MSE evaluation
y_forecasted = pred.predicted_mean
y_truth = series['2000-01-01':]
# Compute the mean square error
MSE = ((y_forecasted - y_truth) ** 2).mean()
print('MSE of the forecasts is {}'.format(round(MSE, 2)))
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={FirstSeasonalDifference.py}, label={FirstSeasonalDifference.py}]
## removing seasonality from time series using seasonal differencing
from pandas import read_excel
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
from matplotlib import pyplot

series = read_excel('Electricity.xls', sheet_name='ELEC', header=0, index_col=0, parse_dates=True, squeeze=True)

# Time, ACF, and PACF plots for original data
pyplot.plot(series)
pyplot.title('Time plot original data')
plot_acf(series, title='ACF plot of original data', lags=50)
plot_pacf(series, title='PACF plot of original data', lags=50)
pyplot.show()

#  Seaonal difference
X = series.values
SeasDiff = list()
for i in range(12, len(X)):
	value = X[i] - X[i - 12]
	SeasDiff.append(value)

# Time, ACF, and PACF plots for the seasonally differenced series
pyplot.plot(SeasDiff)
pyplot.title('Time plot seasonally differenced series')
plot_acf(SeasDiff, title='ACF plot of seasonally differenced series', lags=50)
plot_pacf(SeasDiff, title='PACF plot of seasonally differenced series', lags=50)
pyplot.show()

### Seasonal + First difference
Y = SeasDiff
SeasFirstDiff = list()
for i in range(1, len(Y)):
	value = Y[i] - Y[i - 1]
	SeasFirstDiff.append(value)
pyplot.plot(SeasFirstDiff)
pyplot.title('Time plot seasonally + first differenced series')
plot_acf(SeasFirstDiff, title='ACF plot of seasonally + first differenced series', lags=50)
plot_pacf(SeasFirstDiff, title='PACF plot of seasonally + first differenced series', lags=50)
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={AutomaticOrderSARIMAX.py}, label={AutomaticOrderSARIMAX.py}]
#===================================================
#Code for identifying the parameters with smallest AIC
#===================================================
from pandas import read_excel
import matplotlib.pyplot as plt
import statsmodels.api as sm
import warnings
import itertools
plt.style.use('fivethirtyeight')

series = read_excel('BuildingMaterials.xls', sheet_name='Data', header=0, index_col=0, parse_dates=True, squeeze=True)

#Define the p, d and q parameters to take any value between 0 and 1
p = d = q = range(0, 2)

# Generate all different combinations of p, q and q triplets
pdq = list(itertools.product(p, d, q))

# Generate all different combinations of seasonal p, q and q triplets (i.e., P, D, Q)
seasonal_pdq = [(x[0], x[1], x[2], 12) for x in list(itertools.product(p, d, q))]

# Indentification of best model from different combinations of pdq and seasonal_pdq
warnings.filterwarnings("ignore") # specify to ignore warning messages
best_score, best_param, best_paramSeasonal = float("inf"), None, None
for param in pdq:
    for param_seasonal in seasonal_pdq:
        try:
            mod = sm.tsa.statespace.SARIMAX(series, order=param, seasonal_order=param_seasonal, enforce_invertibility=False)
            results = mod.fit()
            if results.aic < best_score:
                best_score, best_param, best_paramSeasonal = results.aic, param, param_seasonal
            print('ARIMA{}x{} - AIC:{}'.format(param, param_seasonal, results.aic))
        except:
            continue
print('The best model is ARIMA{}x{} - AIC:{}'.format(best_param, best_paramSeasonal, best_score))
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={SARIMAX.py}, label={SARIMAX.py}]
from pandas import read_excel
import pandas as pd
import matplotlib.pyplot as plt
import statsmodels.api as sm
plt.style.use('fivethirtyeight')

#==================================================================
#Loading the data set
df = read_excel('BuildingMaterials.xls', sheet_name='Data', header=0,
                index_col=0, parse_dates=True, squeeze=True)
#==================================================================

#==================================================================
#Fitting the ARIMA model and printing related statistics
# ARIMA(0, 1, 1)(0,1,1)12 in this case;
#this one is based on MA1 model template
mod = sm.tsa.statespace.SARIMAX(df, order=(1,1,1), seasonal_order=(0,1,1,12))
results = mod.fit(disp=False)
print(results.summary())
#==================================================================

#GRAPH BLOCK1======================================================
#Printing the graphical statistics of model (correlogram = ACF plot)
results.plot_diagnostics(figsize=(15, 12))
plt.show()
#==================================================================

#GRAPH BLOCK2======================================================
# printing the part of forecasts fitted to original data (for accuracy evaluation)
# the start date has to be provided; hence should be a time within the original time series;
# in this case, it is to start on 01 January 2000
pred = results.get_prediction(start=pd.to_datetime('2000-01-01'), dynamic=False)
pred_ci = pred.conf_int()

# printing one-step ahead forecasts together with the original data set;
# hence, the starting point (year) of the data set is required
# in order to build the plot of original series
ax = df['1986':].plot(label='Original data')
pred.predicted_mean.plot(ax=ax, label='One-step ahead Forecast', alpha=.7)
ax.fill_between(pred_ci.index,
                pred_ci.iloc[:, 0],
                pred_ci.iloc[:, 1], color='k', alpha=.2)
plt.legend()
plt.show()
#===================================================================

#GRAPH BLOCK3=======================================================
# Get forecast 20 steps ahead in future
pred_uc = results.get_forecast(steps=20)
# Get confidence intervals of forecasts
pred_ci = pred_uc.conf_int()
# plotting forecasts ahead
ax = df.plot(label='Original data')
pred_uc.predicted_mean.plot(ax=ax, label='Forecast values', title='Forecast plot with confidence interval')
ax.fill_between(pred_ci.index,
                pred_ci.iloc[:, 0],
                pred_ci.iloc[:, 1], color='k', alpha=.25)
plt.legend()
plt.show()
#====================================================================

#====================================================================
# MSE evaluation
y_forecasted = pred.predicted_mean
y_truth = df['2000-01-01':]
# Compute the mean square error
MSE = ((y_forecasted - y_truth) ** 2).mean()
print('MSE of the forecasts is {}'.format(round(MSE, 2)))
#====================================================================
\end{lstlisting}

%\begin{lstlisting}[language=Python, caption=Demo 4.3 (ACF + PACF of Dow Jones time series)]
%from pandas import read_excel
%from matplotlib import pyplot
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%series = read_excel('DowJones.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%# ACF plot on 50 time lags
%plot_acf(series, title='ACF of Dow Jones time series', lags=50)
%
%# PACF plot on 50 time lags
%plot_pacf(series, title='PACF of Dow Jones time series', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.4 (Time/ACF/PACF plot Dow Jones 1st difference)]
%## detrend a time series using differencing
%from pandas import read_excel
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%from matplotlib import pyplot
%
%series = read_excel('DowJones.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%X = series.values
%diff = list()
%for i in range(1, len(X)):
%	value = X[i] - X[i - 1]
%	diff.append(value)
%pyplot.plot(diff)
%pyplot.title('Time plot Dow Jones 1st difference')
%
%# ACF plot of time series
%plot_acf(diff, title='ACF of Dow Jones 1st difference', lags=50)
%
%# PACF plot of time series
%plot_pacf(diff, title='PACF of Dow Jones 1st difference', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.5 (Seasonal differencing)]
%from pandas import read_excel
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%from matplotlib import pyplot
%
%series = read_excel('Electricity.xls', sheet_name='ELEC', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%# Time, ACF, and PACF plots for original data
%pyplot.plot(series)
%pyplot.title('Time plot original data')
%plot_acf(series, title='ACF plot of original data', lags=50)
%plot_pacf(series, title='PACF plot of original data', lags=50)
%pyplot.show()
%
%#  Seaonal difference
%X = series.values
%SeasDiff = list()
%for i in range(12, len(X)):
%	value = X[i] - X[i - 12]
%	SeasDiff.append(value)
%
%# Time, ACF, and PACF plots for the seasonally differenced series
%pyplot.plot(SeasDiff)
%pyplot.title('Time plot seasonally differenced series')
%plot_acf(SeasDiff, title='ACF plot of seasonally differenced series', lags=50)
%plot_pacf(SeasDiff, title='PACF plot of seasonally differenced series', lags=50)
%pyplot.show()
%
%### Seasonal + First difference
%Y = SeasDiff
%SeasFirstDiff = list()
%for i in range(1, len(Y)):
%	value = Y[i] - Y[i - 1]
%	SeasFirstDiff.append(value)
%pyplot.plot(SeasFirstDiff)
%pyplot.title('Time plot seasonally + first differenced series')
%plot_acf(SeasFirstDiff, title='ACF plot of seasonally + first differenced series', lags=50)
%plot_pacf(SeasFirstDiff, title='PACF plot of seasonally + first differenced series', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%
%
%
%
%\begin{lstlisting}[language=Python, caption=Demo 4.8--1 (Building an ARIMA model)]
%from pandas import read_excel
%from matplotlib import pyplot
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%series = read_excel('PrintingWriting.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%# ACF plot on 50 time lags
%plot_acf(series, title='ACF printing & writing paper sales', lags=50)
%
%# PACF plot on 50 time lags
%plot_pacf(series, title='PACF printing & writing paper sales', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.8--2 (Building an ARIMA model)]
%## removing seasonality from time series using seasonal differencing
%from pandas import read_excel
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%from matplotlib import pyplot
%
%series = read_excel('PrintingWriting.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%## Time, ACF, and PACF plots for original data
%#pyplot.plot(series)
%#pyplot.title('Time plot original data')
%#plot_acf(series, title='ACF plot of original data', lags=50)
%#plot_pacf(series, title='PACF plot of original data', lags=50)
%#pyplot.show()
%
%#  Seaonal difference
%X = series.values
%SeasDiff = list()
%for i in range(12, len(X)):
%	value = X[i] - X[i - 12]
%	SeasDiff.append(value)
%
%# Time, ACF, and PACF plots for the seasonally differenced series
%pyplot.plot(SeasDiff)
%pyplot.title('Time plot seasonally differenced series')
%plot_acf(SeasDiff, title='ACF plot of seasonally differenced series', lags=50)
%plot_pacf(SeasDiff, title='PACF plot of seasonally differenced series', lags=50)
%pyplot.show()
%
%# Seasonal + First difference
%Y = SeasDiff
%SeasFirstDiff = list()
%for i in range(1, len(Y)):
%	value = Y[i] - Y[i - 1]
%	SeasFirstDiff.append(value)
%pyplot.plot(SeasFirstDiff)
%pyplot.title('Time plot seasonally + first differenced series')
%plot_acf(SeasFirstDiff, title='ACF plot of seasonally + first differenced series', lags=50)
%plot_pacf(SeasFirstDiff, title='PACF plot of seasonally + first differenced series', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.8--3 (Building an ARIMA model)]
%## removing seasonality from time series using seasonal differencing
%from pandas import read_excel
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%from matplotlib import pyplot
%
%series = read_excel('PrintingWriting.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%## Time, ACF, and PACF plots for original data
%#pyplot.plot(series)
%#pyplot.title('Time plot original data')
%#plot_acf(series, title='ACF plot of original data', lags=50)
%#plot_pacf(series, title='PACF plot of original data', lags=50)
%#pyplot.show()
%
%#  Seaonal difference
%X = series.values
%SeasDiff = list()
%for i in range(12, len(X)):
%	value = X[i] - X[i - 12]
%	SeasDiff.append(value)
%
%# Time, ACF, and PACF plots for the seasonally differenced series
%pyplot.plot(SeasDiff)
%pyplot.title('Time plot seasonally differenced series')
%plot_acf(SeasDiff, title='ACF plot of seasonally differenced series', lags=50)
%plot_pacf(SeasDiff, title='PACF plot of seasonally differenced series', lags=50)
%pyplot.show()
%
%#### Seasonal + First difference
%#Y = SeasDiff
%#SeasFirstDiff = list()
%#for i in range(1, len(Y)):
%#	value = Y[i] - Y[i - 1]
%#	SeasFirstDiff.append(value)
%#pyplot.plot(SeasFirstDiff)
%#pyplot.title('Time plot seasonally + first differenced series')
%#plot_acf(SeasFirstDiff, title='ACF plot of seasonally + first differenced series', lags=50)
%#plot_pacf(SeasFirstDiff, title='PACF plot of seasonally + first differenced series', lags=50)
%#pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.8--4 (Building an ARIMA model)]
%from pandas import read_excel
%import pandas as pd
%import matplotlib.pyplot as plt
%import statsmodels.api as sm
%plt.style.use('fivethirtyeight')
%
%###############################
%df = read_excel('PrintingWriting.xls', sheet_name='Data2', header=0,
%               index_col=0, parse_dates=True, squeeze=True)
%
%# ARIMA model with (p, d, q)=(1, 1, 1)
%#mod = sm.tsa.statespace.SARIMAX(df, trend='c', order=(1,1,1))
%mod = sm.tsa.statespace.SARIMAX(df, order=(1,1,1),
%                                seasonal_order=(1,1,1,12))
%results = mod.fit(disp=False)
%print(results.summary())
%
%# graphical statistics of model (correlogram = ACF plot)
%results.plot_diagnostics(figsize=(15, 12))
%plt.show()
%
%#============================================
%# this code requires the fitted forecasts (for accuracy evaluation) to start 01 Jan 1979.
%pred = results.get_prediction(start=pd.to_datetime('1972-01-01'), dynamic=False)
%pred_ci = pred.conf_int()
%
%print(pred_ci)
%
%# this code requires the whole plot to start in 1956 (start year of data)
%ax = df['1969':].plot(label='Original data')
%pred.predicted_mean.plot(ax=ax, label='One-step ahead Forecast', alpha=.7)
%
%ax.fill_between(pred_ci.index,
%                pred_ci.iloc[:, 0],
%                pred_ci.iloc[:, 1], color='k', alpha=.2)
%plt.legend()
%plt.show()
%#=============================================
%# MSE evaluation
%y_forecasted = pred.predicted_mean
%y_truth = df['1965-01-01':]
%# Compute the mean square error
%mse = ((y_forecasted - y_truth) ** 2).mean()
%print('MSE of the forecasts is {}'.format(round(mse, 2)))
%
%#=============================================
%# get forecast 20 steps ahead in future
%pred_uc = results.get_forecast(steps=20)
%# Get confidence intervals of forecasts
%pred_ci = pred_uc.conf_int()
%
%# plotting forecasts ahead
%ax = df.plot(label='Original data')
%pred_uc.predicted_mean.plot(ax=ax, label='Forecast values', title='Forecast plot with confidence interval')
%ax.fill_between(pred_ci.index,
%                pred_ci.iloc[:, 0],
%                pred_ci.iloc[:, 1], color='k', alpha=.25)
%plt.legend()
%plt.show()
%#----------------------------------------------
%\end{lstlisting}

\section{Codes on the regression analysis and application to forecasting}

%\begin{lstlisting}[language=Python, caption={RegressionTimePlot.py}, label={RegressionTimePlot.py}]
%from pandas import read_excel
%import matplotlib.pyplot as plt
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%DEOM.plot()
%plt.xlabel('time')
%plt.ylabel('Difference end of month balance')
%plt.title('DEOM')
%plt.show()
%
%AAA.plot()
%plt.xlabel('time')
%plt.ylabel('Composite AAA Bond rates')
%plt.title('AAA')
%plt.show()
%
%Tto4.plot()
%plt.xlabel('time')
%plt.ylabel('US Govt 3-4 year Bond rates')
%plt.title('3to4')
%plt.show()
%
%D3to4.plot()
%plt.xlabel('time')
%plt.ylabel('Difference US Govt 3-4 year Bond rates')
%plt.title('D3to4')
%plt.show()
%\end{lstlisting}



\begin{lstlisting}[language=Python, caption={RegressionAnalysis.py}, label={Regression.py}]
from pandas import read_excel
from statsmodels.formula.api import ols
series = read_excel('Bank.xls', sheet_name='Data2', header=0,
                     squeeze=True, dtype=float)

#reading the basic variables
DEOM = series.DEOM
AAA = series.AAA
Tto4 = series.Tto4
D3to4 = series.D3to4

#Regression model(s)
formula = 'DEOM ~ AAA + Tto4 + D3to4'

#Ordinary Least Squares (OLS)
results = ols(formula, data=series).fit()
print(results.summary())

# Here the main table is the first one,
# where the main statistics are the R-squared (line 1)
# and the P-value; i.e., Prob (F-statistic)
\end{lstlisting}


%\begin{lstlisting}[language=Python, caption=Demo 3.3 (Individual significance analysis)]
%from pandas import read_excel
%from statsmodels.formula.api import ols
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%#Regression model(s)
%formula = 'DEOM ~ AAA + Tto4 + D3to4'
%
%#Ordinary Least Squares (OLS)
%results = ols(formula, data=series).fit()
%print(results.summary())
%
%# Here the main table is the second one,
%# where all the statistics of the individual variables
%# are given.
%\end{lstlisting}
%
%
%\begin{lstlisting}[language=Python, caption=Demo 3.4 (Statistics for model with indicator variables)]
%from pandas import read_excel
%from statsmodels.formula.api import ols
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%#reading the indicator variables
%D1=series.D1
%D2=series.D2
%D3=series.D3
%D4=series.D4
%D5=series.D5
%D6=series.D6
%D7=series.D7
%D8=series.D8
%D9=series.D9
%D10=series.D10
%D11=series.D11
%
%#Regression model(s)
%formula = 'DEOM ~ AAA + Tto4 + D3to4 + D1 + D2 + D3+D4+D5+D6+D7+D8+D9+D10+D11'
%
%
%#Ordinary Least Squares (OLS)
%results = ols(formula, data=series).fit()
%print(results.summary())
%
%# the two tables show the changes in the overall and
%# individual significance of the model when
%# the indicator variables (Di, i=1, ..., 11) are added
%# Pay attention to the changes in the key statistics
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 3.5 (Statistics for model with indicator + time variables)]
%from pandas import read_excel
%from statsmodels.formula.api import ols
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%#reading the indicator variables
%D1=series.D1
%D2=series.D2
%D3=series.D3
%D4=series.D4
%D5=series.D5
%D6=series.D6
%D7=series.D7
%D8=series.D8
%D9=series.D9
%D10=series.D10
%D11=series.D11
%
%#reading the time variable
%time=series.time
%
%#Regression model(s)
%formula = 'DEOM ~ AAA + Tto4 + D3to4 + D1 + D2 + D3+D4+D5+D6+D7+D8+D9+D10+D11+time'
%
%#Ordinary Least Squares (OLS)
%results = ols(formula, data=series).fit()
%print(results.summary())
%
%# the difference with what is done
%# in StatsWithIndicatorsBank.py is the addition of time
%# So the same statistics remain important to see the changes
%\end{lstlisting}
%
%
%\begin{lstlisting}[language=Python, caption=Demo 3.6 (Statistics comparision)]
%from pandas import read_excel
%from statsmodels.formula.api import ols
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%#reading the indicator variables
%D1=series.D1
%D2=series.D2
%D3=series.D3
%D4=series.D4
%D5=series.D5
%D6=series.D6
%D7=series.D7
%D8=series.D8
%D9=series.D9
%D10=series.D10
%D11=series.D11
%
%#reading the time variable
%time=series.time
%
%#Regression model(s)
%formula1 = 'DEOM ~ AAA + Tto4 + D3to4'
%formula2 = 'DEOM ~ AAA + Tto4 + D3to4 + D1 + D2 + D3+D4+D5+D6+D7+D8+D9+D10+D11'
%formula3 = 'DEOM ~ AAA + Tto4 + D3to4 + D1 + D2 + D3+D4+D5+D6+D7+D8+D9+D10+D11+time'
%
%#Ordinary Least Squares (OLS)
%results1 = ols(formula1, data=series).fit()
%results2 = ols(formula2, data=series).fit()
%results3 = ols(formula3, data=series).fit()
%print(results1.summary())
%print(results2.summary())
%print(results3.summary())
%
%# the results from IndividualSignificance.py,
%# StatsWithIndicatorsBank.py,
%# and StatsWithIndicatorsTimeBank.py are summarised
%# for easy comparison of the key statistics
%\end{lstlisting}


\begin{lstlisting}[language=Python, caption={RegressionForecast.py}, label={RegressionForecast.py}]
from pandas import read_excel
from statsmodels.tsa.api import Holt
#from matplotlib import pyplot
import matplotlib.pyplot as plt
import numpy as np
from statsmodels.formula.api import ols
series = read_excel('Bank.xls', sheet_name='Data2', header=0,
                     squeeze=True, dtype=float)

# Reading the basic variables
DEOM = series.DEOM
AAA = series.AAA
Tto4 = series.Tto4
D3to4 = series.D3to4

# Forecasting for AAA using Holt's linear method
fit1 = Holt(AAA).fit(optimized=True)
fcast1 = fit1.forecast(6).rename("Additive 2 damped trend")
fit1.fittedvalues.plot(color='red')
fcast1.plot(color='red', legend=True)
AAA.plot(color='black', legend=True)
plt.title('Forecast of AAA with Holt linear method')
plt.show()

# Forecasting for Tto4 using Holt's linear method
fit2 = Holt(Tto4).fit(optimized=True)
fcast2 = fit2.forecast(6).rename("Additive 2 damped trend")
fit2.fittedvalues.plot(color='red')
fcast2.plot(color='red', legend=True)
Tto4.plot(color='black', legend=True)
plt.title('Forecast of 3to4 with Holt linear method')
plt.show()

# Forecasting for D3to4 using Holt's linear method
fit3 = Holt(D3to4).fit(smoothing_level=0.8, smoothing_slope=0.2, optimized=False)
#fit3 = Holt(D3to4).fit(optimized=True)
fcast3 = fit3.forecast(6).rename("Additive 2 damped trend")
fit3.fittedvalues.plot(color='red')
fcast3.plot(color='red', legend=True)
D3to4.plot(color='black', legend=True)
plt.title('Forecast of D3to4 with Holt linear method')
plt.show()

# Building the regression based forecast for main variable, DEOM
# Regression model(s)
formula = 'DEOM ~ AAA + Tto4 + D3to4'

# ols generate statistics and the parameters b0, b1, etc., of the model
results = ols(formula, data=series).fit()
results.summary()
b0 = results.params.Intercept
b1 = results.params.AAA
b2 = results.params.Tto4
b3 = results.params.D3to4

# putting the fitted values of the forecasts of AAA, Tto4, and D3to4 in arrays
a1 = np.array(fit1.fittedvalues)
a2 = np.array(fit2.fittedvalues)
a3 = np.array(fit3.fittedvalues)

# Building the fitted part of the forecast of DEOM
F=a1
for i in range(53):
    F[i] = b0 + a1[i]*b1 + a2[i]*b2 + a3[i]*b3

# putting the values of the forecasts of AAA, Tto4, and D3to4 in arrays
v1=np.array(fcast1)
v2=np.array(fcast2)
v3=np.array(fcast3)

# Building the 6 values of the forecast ahead
E=v1
for i in range(6):
    E[i] = b0 + v1[i]*b1 + v2[i]*b2 + v3[i]*b3


# Joining the fitted values of the forecast and the points ahead
K=np.append(F, E)

# Reading the original DEOM time series for all the 59 periods
DEOMfull0 = read_excel('Bank.xls', sheet_name='Data4', header=0,
                     squeeze=True, dtype=float)

###########################
# Evaluating the MSE to generate the confidence interval
DEOMfull = DEOMfull0.DEOMfull
values=DEOMfull[0:53]
Error = values - F
MSE=sum(Error**2)*1.0/len(F)

## Lower and upper bounds of forecasts for z=1.282; see equation (2.2) in Chap 2.
#LowerE = E - 1.282*MSE
#UpperE = E + 1.282*MSE

LowerE = DEOMfull0.LowerE
UpperE = DEOMfull0.UpperE

print(LowerE)
###############################

# Plotting the graphs of K and DEOMfull with legends
from matplotlib.legend_handler import HandlerLine2D
line1, = plt.plot(K, color='red', label='Forecast values')
line2, = plt.plot(DEOMfull, color='black', label='Original data')
line3, = plt.plot(LowerE, color='blue', label='Lower forecast')
line4, = plt.plot(UpperE, color='orange', label='Upper forecast')
plt.legend(handler_map={line1: HandlerLine2D(numpoints=4)})
plt.title('DEOM regression forecast with confidence interval')
plt.show()

# Proceeding as as in other demos, forecasts
# can be generated for other scenarios; i.e., with different combinations of variables
\end{lstlisting}


==> Source file of paper - final/structure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The Legrand Orange Book
% Structural Definitions File
% Version 2.0 (9/2/15)
%
% Original author:
% Mathias Legrand (legrand.mathias@gmail.com) with modifications by:
% Vel (vel@latextemplates.com)
% 
% This file has been downloaded from:
% http://www.LaTeXTemplates.com
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	VARIOUS REQUIRED PACKAGES AND CONFIGURATIONS
%----------------------------------------------------------------------------------------

\usepackage[top=3cm,bottom=3cm,left=3cm,right=3cm,headsep=10pt,a4paper]{geometry} % Page margins

\usepackage{graphicx} % Required for including pictures
\graphicspath{{Pictures/}} % Specifies the directory where pictures are stored

\usepackage{lipsum} % Inserts dummy text

\usepackage{tikz} % Required for drawing custom shapes

\usepackage[english]{babel} % English language/hyphenation

\usepackage{enumitem} % Customize lists
\setlist{nolistsep} % Reduce spacing between bullet points and numbered lists

\usepackage{booktabs} % Required for nicer horizontal rules in tables

\usepackage{xcolor} % Required for specifying colors by name
\definecolor{ocre}{RGB}{243,102,25} % Define the orange color used for highlighting throughout the book

%----------------------------------------------------------------------------------------
%	FONTS
%----------------------------------------------------------------------------------------

\usepackage{avant} % Use the Avantgarde font for headings
%\usepackage{times} % Use the Times font for headings
\usepackage{mathptmx} % Use the Adobe Times Roman as the default text font together with math symbols from the Sym­bol, Chancery and Com­puter Modern fonts

\usepackage{microtype} % Slightly tweak font spacing for aesthetics
\usepackage[utf8]{inputenc} % Required for including letters with accents
\usepackage[T1]{fontenc} % Use 8-bit encoding that has 256 glyphs

%----------------------------------------------------------------------------------------
%	BIBLIOGRAPHY AND INDEX
%----------------------------------------------------------------------------------------

\usepackage[style=alphabetic,citestyle=numeric,sorting=nyt,sortcites=true,autopunct=true,babel=hyphen,hyperref=true,abbreviate=false,backref=true,backend=biber]{biblatex}
\addbibresource{bibliography.bib} % BibTeX bibliography file
\defbibheading{bibempty}{}

\usepackage{calc} % For simpler calculation - used for spacing the index letter headings correctly
\usepackage{makeidx} % Required to make an index
\makeindex % Tells LaTeX to create the files required for indexing

%----------------------------------------------------------------------------------------
%	MAIN TABLE OF CONTENTS
%----------------------------------------------------------------------------------------

\usepackage{titletoc} % Required for manipulating the table of contents

\contentsmargin{0cm} % Removes the default margin

% Part text styling
\titlecontents{part}[0cm]
{\addvspace{20pt}\centering\large\bfseries}
{}
{}
{}

% Chapter text styling
\titlecontents{chapter}[1.25cm] % Indentation
{\addvspace{12pt}\large\sffamily\bfseries} % Spacing and font options for chapters
{\color{ocre!60}\contentslabel[\Large\thecontentslabel]{1.25cm}\color{ocre}} % Chapter number
{\color{ocre}}  
{\color{ocre!60}\normalsize\;\titlerule*[.5pc]{.}\;\thecontentspage} % Page number

% Section text styling
\titlecontents{section}[1.25cm] % Indentation
{\addvspace{3pt}\sffamily\bfseries} % Spacing and font options for sections
{\contentslabel[\thecontentslabel]{1.25cm}} % Section number
{}
{\hfill\color{black}\thecontentspage} % Page number
[]

% Subsection text styling
\titlecontents{subsection}[1.25cm] % Indentation
{\addvspace{1pt}\sffamily\small} % Spacing and font options for subsections
{\contentslabel[\thecontentslabel]{1.25cm}} % Subsection number
{}
{\ \titlerule*[.5pc]{.}\;\thecontentspage} % Page number
[]

% List of figures
\titlecontents{figure}[0em]
{\addvspace{-5pt}\sffamily}
{\thecontentslabel\hspace*{1em}}
{}
{\ \titlerule*[.5pc]{.}\;\thecontentspage}
[]

% List of tables
\titlecontents{table}[0em]
{\addvspace{-5pt}\sffamily}
{\thecontentslabel\hspace*{1em}}
{}
{\ \titlerule*[.5pc]{.}\;\thecontentspage}
[]

%----------------------------------------------------------------------------------------
%	MINI TABLE OF CONTENTS IN PART HEADS
%----------------------------------------------------------------------------------------

% Chapter text styling
\titlecontents{lchapter}[0em] % Indenting
{\addvspace{15pt}\large\sffamily\bfseries} % Spacing and font options for chapters
{\color{ocre}\contentslabel[\Large\thecontentslabel]{1.25cm}\color{ocre}} % Chapter number
{}  
{\color{ocre}\normalsize\sffamily\bfseries\;\titlerule*[.5pc]{.}\;\thecontentspage} % Page number

% Section text styling
\titlecontents{lsection}[0em] % Indenting
{\sffamily\small} % Spacing and font options for sections
{\contentslabel[\thecontentslabel]{1.25cm}} % Section number
{}
{}

% Subsection text styling
\titlecontents{lsubsection}[.5em] % Indentation
{\normalfont\footnotesize\sffamily} % Font settings
{}
{}
{}

%----------------------------------------------------------------------------------------
%	PAGE HEADERS
%----------------------------------------------------------------------------------------

\usepackage{fancyhdr} % Required for header and footer configuration

\pagestyle{fancy}
\renewcommand{\chaptermark}[1]{\markboth{\sffamily\normalsize\bfseries\chaptername\ \thechapter.\ #1}{}} % Chapter text font settings
\renewcommand{\sectionmark}[1]{\markright{\sffamily\normalsize\thesection\hspace{5pt}#1}{}} % Section text font settings
\fancyhf{} \fancyhead[LE,RO]{\sffamily\normalsize\thepage} % Font setting for the page number in the header
\fancyhead[LO]{\rightmark} % Print the nearest section name on the left side of odd pages
\fancyhead[RE]{\leftmark} % Print the current chapter name on the right side of even pages
\renewcommand{\headrulewidth}{0.5pt} % Width of the rule under the header
\addtolength{\headheight}{2.5pt} % Increase the spacing around the header slightly
\renewcommand{\footrulewidth}{0pt} % Removes the rule in the footer
\fancypagestyle{plain}{\fancyhead{}\renewcommand{\headrulewidth}{0pt}} % Style for when a plain pagestyle is specified

% Removes the header from odd empty pages at the end of chapters
\makeatletter
\renewcommand{\cleardoublepage}{
\clearpage\ifodd\c@page\else
\hbox{}
\vspace*{\fill}
\thispagestyle{empty}
\newpage
\fi}

%----------------------------------------------------------------------------------------
%	THEOREM STYLES
%----------------------------------------------------------------------------------------

\usepackage{amsmath,amsfonts,amssymb,amsthm} % For math equations, theorems, symbols, etc

\newcommand{\intoo}[2]{\mathopen{]}#1\,;#2\mathclose{[}}
\newcommand{\ud}{\mathop{\mathrm{{}d}}\mathopen{}}
\newcommand{\intff}[2]{\mathopen{[}#1\,;#2\mathclose{]}}
\newtheorem{notation}{Notation}[chapter]

% Boxed/framed environments
\newtheoremstyle{ocrenumbox}% % Theorem style name
{0pt}% Space above
{0pt}% Space below
{\normalfont}% % Body font
{}% Indent amount
{\small\bf\sffamily\color{ocre}}% % Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\color{ocre}\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries\color{black}---\nobreakspace#3.}} % Optional theorem note
\renewcommand{\qedsymbol}{$\blacksquare$}% Optional qed square

\newtheoremstyle{blacknumex}% Theorem style name
{5pt}% Space above
{5pt}% Space below
{\normalfont}% Body font
{} % Indent amount
{\small\bf\sffamily}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily{\tiny\ensuremath{\blacksquare}}\nobreakspace\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries---\nobreakspace#3.}}% Optional theorem note

\newtheoremstyle{blacknumbox} % Theorem style name
{0pt}% Space above
{0pt}% Space below
{\normalfont}% Body font
{}% Indent amount
{\small\bf\sffamily}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries---\nobreakspace#3.}}% Optional theorem note

% Non-boxed/non-framed environments
\newtheoremstyle{ocrenum}% % Theorem style name
{5pt}% Space above
{5pt}% Space below
{\normalfont}% % Body font
{}% Indent amount
{\small\bf\sffamily\color{ocre}}% % Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\color{ocre}\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries\color{black}---\nobreakspace#3.}} % Optional theorem note
\renewcommand{\qedsymbol}{$\blacksquare$}% Optional qed square
\makeatother

% Defines the theorem text style for each type of theorem to one of the three styles above
\newcounter{dummy} 
\numberwithin{dummy}{section}
\theoremstyle{ocrenumbox}
\newtheorem{theoremeT}[dummy]{Theorem}
\newtheorem{problem}{Problem}[chapter]
\newtheorem{exerciseT}{Exercise}[chapter]
\theoremstyle{blacknumex}
\newtheorem{exampleT}{Example}[chapter]
\theoremstyle{blacknumbox}
\newtheorem{vocabulary}{Vocabulary}[chapter]
\newtheorem{definitionT}{Definition}[section]
\newtheorem{corollaryT}[dummy]{Corollary}
\theoremstyle{ocrenum}
\newtheorem{proposition}[dummy]{Proposition}

%----------------------------------------------------------------------------------------
%	DEFINITION OF COLORED BOXES
%----------------------------------------------------------------------------------------

\RequirePackage[framemethod=default]{mdframed} % Required for creating the theorem, definition, exercise and corollary boxes

% Theorem box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
backgroundcolor=black!5,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
innerbottommargin=5pt]{tBox}

% Exercise box	  
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
backgroundcolor=ocre!10,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
innerbottommargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt]{eBox}	

% Definition box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=0pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt,
innerbottommargin=0pt]{dBox}	

% Corollary box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
linecolor=gray,
backgroundcolor=black!5,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt,
innerbottommargin=5pt]{cBox}

% Creates an environment for each type of theorem and assigns it a theorem text style from the "Theorem Styles" section above and a colored box from above
\newenvironment{theorem}{\begin{tBox}\begin{theoremeT}}{\end{theoremeT}\end{tBox}}
\newenvironment{exercise}{\begin{eBox}\begin{exerciseT}}{\hfill{\color{ocre}\tiny\ensuremath{\blacksquare}}\end{exerciseT}\end{eBox}}				  
\newenvironment{definition}{\begin{dBox}\begin{definitionT}}{\end{definitionT}\end{dBox}}	
\newenvironment{example}{\begin{exampleT}}{\hfill{\tiny\ensuremath{\blacksquare}}\end{exampleT}}		
\newenvironment{corollary}{\begin{cBox}\begin{corollaryT}}{\end{corollaryT}\end{cBox}}	

%----------------------------------------------------------------------------------------
%	REMARK ENVIRONMENT
%----------------------------------------------------------------------------------------

\newenvironment{remark}{\par\vspace{10pt}\small % Vertical white space above the remark and smaller font size
\begin{list}{}{
\leftmargin=35pt % Indentation on the left
\rightmargin=25pt}\item\ignorespaces % Indentation on the right
\makebox[-2.5pt]{\begin{tikzpicture}[overlay]
\node[draw=ocre!60,line width=1pt,circle,fill=ocre!25,font=\sffamily\bfseries,inner sep=2pt,outer sep=0pt] at (-15pt,0pt){\textcolor{ocre}{R}};\end{tikzpicture}} % Orange R in a circle
\advance\baselineskip -1pt}{\end{list}\vskip5pt} % Tighter line spacing and white space after remark

%----------------------------------------------------------------------------------------
%	SECTION NUMBERING IN THE MARGIN
%----------------------------------------------------------------------------------------

\makeatletter
\renewcommand{\@seccntformat}[1]{\llap{\textcolor{ocre}{\csname the#1\endcsname}\hspace{1em}}}                    
\renewcommand{\section}{\@startsection{section}{1}{\z@}
{-4ex \@plus -1ex \@minus -.4ex}
{1ex \@plus.2ex }
{\normalfont\large\sffamily\bfseries}}
\renewcommand{\subsection}{\@startsection {subsection}{2}{\z@}
{-3ex \@plus -0.1ex \@minus -.4ex}
{0.5ex \@plus.2ex }
{\normalfont\sffamily\bfseries}}
\renewcommand{\subsubsection}{\@startsection {subsubsection}{3}{\z@}
{-2ex \@plus -0.1ex \@minus -.2ex}
{.2ex \@plus.2ex }
{\normalfont\small\sffamily\bfseries}}                        
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}
{-2ex \@plus-.2ex \@minus .2ex}
{.1ex}
{\normalfont\small\sffamily\bfseries}}

%----------------------------------------------------------------------------------------
%	PART HEADINGS
%----------------------------------------------------------------------------------------

% numbered part in the table of contents
\newcommand{\@mypartnumtocformat}[2]{%
\setlength\fboxsep{0pt}%
\noindent\colorbox{ocre!20}{\strut\parbox[c][.7cm]{\ecart}{\color{ocre!70}\Large\sffamily\bfseries\centering#1}}\hskip\esp\colorbox{ocre!40}{\strut\parbox[c][.7cm]{\linewidth-\ecart-\esp}{\Large\sffamily\centering#2}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% unnumbered part in the table of contents
\newcommand{\@myparttocformat}[1]{%
\setlength\fboxsep{0pt}%
\noindent\colorbox{ocre!40}{\strut\parbox[c][.7cm]{\linewidth}{\Large\sffamily\centering#1}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength\esp
\setlength\esp{4pt}
\newlength\ecart
\setlength\ecart{1.2cm-\esp}
\newcommand{\thepartimage}{}%
\newcommand{\partimage}[1]{\renewcommand{\thepartimage}{#1}}%
\def\@part[#1]#2{%
\ifnum \c@secnumdepth >-2\relax%
\refstepcounter{part}%
\addcontentsline{toc}{part}{\texorpdfstring{\protect\@mypartnumtocformat{\thepart}{#1}}{\partname~\thepart\ ---\ #1}}
\else%
\addcontentsline{toc}{part}{\texorpdfstring{\protect\@myparttocformat{#1}}{#1}}%
\fi%
\startcontents%
\markboth{}{}%
{\thispagestyle{empty}%
\begin{tikzpicture}[remember picture,overlay]%
\node at (current page.north west){\begin{tikzpicture}[remember picture,overlay]%	
\fill[ocre!20](0cm,0cm) rectangle (\paperwidth,-\paperheight);
\node[anchor=north] at (4cm,-3.25cm){\color{ocre!40}\fontsize{220}{100}\sffamily\bfseries\@Roman\c@part}; 
\node[anchor=south east] at (\paperwidth-1cm,-\paperheight+1cm){\parbox[t][][t]{8.5cm}{
\printcontents{l}{0}{\setcounter{tocdepth}{1}}%
}};
\node[anchor=north east] at (\paperwidth-1.5cm,-3.25cm){\parbox[t][][t]{15cm}{\strut\raggedleft\color{white}\fontsize{30}{30}\sffamily\bfseries#2}};
\end{tikzpicture}};
\end{tikzpicture}}%
\@endpart}
\def\@spart#1{%
\startcontents%
\phantomsection
{\thispagestyle{empty}%
\begin{tikzpicture}[remember picture,overlay]%
\node at (current page.north west){\begin{tikzpicture}[remember picture,overlay]%	
\fill[ocre!20](0cm,0cm) rectangle (\paperwidth,-\paperheight);
\node[anchor=north east] at (\paperwidth-1.5cm,-3.25cm){\parbox[t][][t]{15cm}{\strut\raggedleft\color{white}\fontsize{30}{30}\sffamily\bfseries#1}};
\end{tikzpicture}};
\end{tikzpicture}}
\addcontentsline{toc}{part}{\texorpdfstring{%
\setlength\fboxsep{0pt}%
\noindent\protect\colorbox{ocre!40}{\strut\protect\parbox[c][.7cm]{\linewidth}{\Large\sffamily\protect\centering #1\quad\mbox{}}}}{#1}}%
\@endpart}
\def\@endpart{\vfil\newpage
\if@twoside
\if@openright
\null
\thispagestyle{empty}%
\newpage
\fi
\fi
\if@tempswa
\twocolumn
\fi}

%----------------------------------------------------------------------------------------
%	CHAPTER HEADINGS
%----------------------------------------------------------------------------------------

% A switch to conditionally include a picture, implemented by  Christian Hupfer
\newif\ifusechapterimage
\usechapterimagetrue
\newcommand{\thechapterimage}{}%
\newcommand{\chapterimage}[1]{\ifusechapterimage\renewcommand{\thechapterimage}{#1}\fi}%
\def\@makechapterhead#1{%
{\parindent \z@ \raggedright \normalfont
\ifnum \c@secnumdepth >\m@ne
\if@mainmatter
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}\thechapter. #1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\else
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}#1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\fi\fi\par\vspace*{270\p@}}}

%-------------------------------------------

\def\@makeschapterhead#1{%
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}#1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\par\vspace*{270\p@}}
\makeatother

%----------------------------------------------------------------------------------------
%	HYPERLINKS IN THE DOCUMENTS
%----------------------------------------------------------------------------------------

\usepackage{hyperref}
\hypersetup{hidelinks,backref=true,pagebackref=true,hyperindex=true,colorlinks=false,breaklinks=true,urlcolor= ocre,bookmarks=true,bookmarksopen=false,pdftitle={Title},pdfauthor={Author}}
\usepackage{bookmark}
\bookmarksetup{
open,
numbered,
addtohook={%
\ifnum\bookmarkget{level}=0 % chapter
\bookmarksetup{bold}%
\fi
\ifnum\bookmarkget{level}=-1 % part
\bookmarksetup{color=ocre,bold}%
\fi
}
}


==> appendices.tex <==
\appendix

\section{Codes on preliminaries on python and data analysis}


\begin{lstlisting}[language=Python, caption={TimePlot}, label={TimePlot}]
from pandas import read_excel
from matplotlib import pyplot
series = read_excel('ClayBricks.xls', sheetname='BRICKSQ', header=0,
              index_col=0, parse_dates=True, squeeze=True)
series.plot()
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={SeasonalPlot}, label={SeasonalPlot}]
from pandas import read_excel
import matplotlib.pyplot as plt
import numpy as np
series = read_excel('ClayBricks.xls',
              sheetname='SeasonalData', header=0, index_col=0, parse_dates=True, squeeze=True)
x = np.array([0,1,2,3,4,5,6,7,8,9,10,11])
months = ['Jan','Feb','Mar','Apr', 'May', 'Jun', 'Jul', 'Aug', 'Sep', 'Oct', 'Nov', 'Dec']
plt.xticks(x, months)
plt.plot(x, series)
plt.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={LogTransform}, label={LogTransform}]
from pandas import read_excel
from pandas import DataFrame
from numpy import log
from matplotlib import pyplot
series = read_excel('Electricity.xls',
              sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
dataframe = DataFrame(series.values)
dataframe.columns = ['electricity']
dataframe['electricity'] = log(dataframe['electricity'])
pyplot.figure(1)
# line plot
pyplot.subplot(211)
pyplot.plot(dataframe['electricity'])
# histogram
pyplot.subplot(212)
pyplot.hist(dataframe['electricity'])
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={SqrtTransform}, label={SqrtTransform}]
from pandas import read_excel
from pandas import DataFrame
from numpy import sqrt
from matplotlib import pyplot
series = read_excel('Electricity.xls',
              sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
dataframe = DataFrame(series.values)
dataframe.columns = ['electricity']
dataframe['electricity'] = sqrt(dataframe['electricity'])
pyplot.figure(1)
# line plot
pyplot.subplot(211)
pyplot.plot(dataframe['electricity'])
# histogram
pyplot.subplot(212)
pyplot.hist(dataframe['electricity'])
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={CalendarAdjustment}, label={CalendarAdjustment}]
from pandas import read_excel
from matplotlib import pyplot
series = read_excel('MilkProduction.xls',
              sheetname='AdjustedData', header=0,
              index_col=0, parse_dates=True, squeeze=True)  # you can include various other parameters
series.plot()
pyplot.show()
\end{lstlisting}




%\begin{lstlisting}[language=Python, caption=Demo 1.3 (code plotting the scatter plot for the used cars vs their current milleage)]
%import pandas as pd
%import matplotlib.pyplot as plt
%#import numpy as np
%from pandas import read_excel
%series1 = read_excel('JapaneseCars.xls', sheet_name='Data', usecols = [0], header=0,
%                     squeeze=True, dtype=float)
%series2 = read_excel('JapaneseCars.xls', sheet_name='Data', usecols=[1], header=0,
%                     squeeze=True, dtype=float)
%
%Japanese = {'Mileage': series1, 'Price': series2}
%df = pd.DataFrame(Japanese, columns=['Mileage', 'Price'])
%plt.scatter(df.Mileage, df.Price)
%
%plt.xlabel('Mileage (MPG)')
%plt.ylabel('Price (US$)')
%plt.title('Price/Mileage Relationship for 19 Japanese cars')
%\end{lstlisting}


\begin{lstlisting}[language=Python,  caption={Correlation}, label={correlation}]
from pandas import read_excel
import numpy as np
series1 = read_excel('JapaneseCars.xls', sheet_name='Data', usecols = [0], header=0,
                     squeeze=True, dtype=float)
series2 = read_excel('JapaneseCars.xls', sheet_name='Data', usecols=[1], header=0,
                     squeeze=True, dtype=float)
correlval=np.corrcoef(series1, series2)
correlval=correlval[1,0]
print(correlval)
\end{lstlisting}

%\begin{lstlisting}[language=Python, caption=Demo 1.5 (Calculating/plotting/representing the autocorrelation), label={autocorrelation1}]
%# create an autocorrelation plot
%from pandas import read_excel
%from matplotlib import pyplot
%from pandas.plotting import autocorrelation_plot
%series = read_excel('Beer.xls', sheet_name='Data', header=0, index_col=0, parse_dates=True, squeeze=True)
%autocorrelation_plot(series)
%pyplot.show()
%\end{lstlisting}
%
%
%\begin{lstlisting}[language=Python, caption=Demo 1.6 (Trend estimation/calculation/representation)]
%from pandas import read_excel
%from matplotlib import pyplot
%series = read_excel('HouseSales.xls',
%              sheetname='MAData', header=0,
%              index_col=0, parse_dates=True, squeeze=True)  # you can include various other parameters
%series.plot()
%pyplot.show()
%\end{lstlisting}
%
\begin{lstlisting}[language=Python, caption={DecompositionAdditive}, label={DecompositionAdditive}]
from pandas import read_excel
from matplotlib import pyplot
from statsmodels.tsa.seasonal import seasonal_decompose
series = read_excel('HouseSales.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
result = seasonal_decompose(series, model='additive')
#result = seasonal_decompose(series, model='multiplicative')
result.plot()
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={DecompositionMultiplicative}, label={DecompositionMultiplicative}]
from pandas import read_excel
from matplotlib import pyplot
from statsmodels.tsa.seasonal import seasonal_decompose
series = read_excel('AirlineSales.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
#result = seasonal_decompose(series, model='additive')
result = seasonal_decompose(series, model='multiplicative')
result.plot()
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={CorrelationMatrix}, label={CorrelationMatrix}]
from pandas import read_excel
import matplotlib.pyplot as plt
import pandas as pd
series = read_excel('Bank.xls', sheet_name='Data3', header=0,
                     squeeze=True, dtype=float)

#Plotting the scatter plots of each variable against the other one
pd.plotting.scatter_matrix(series, figsize=(8, 8))
plt.show()

# Correlation matrix for all the variables, 2 by 2
CorrelationMatrix = series.corr()
print(CorrelationMatrix)
# As in the case of Demo 1.4, corrcoef can be used for the variables in couples.
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={Autocorrelation}, label={Autocorrelation}]
from pandas import read_excel
from matplotlib import pyplot
from pandas.plotting import autocorrelation_plot
from statsmodels.graphics.tsaplots import plot_acf
series1 = read_excel('CementProduction.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
series2 = read_excel('CementProduction.xls', sheetname='SeasonalData', header=0,
                    index_col=0, parse_dates=True, squeeze=True)
series2.plot(title='Seasonal plots building materials time series')
pyplot.show()

plot_acf(series1, title='ACF plot of building materials time series', lags=60)
pyplot.show()

autocorrelation_plot(series1)
pyplot.show()
\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Codes on exponential smoothing methods}

\begin{lstlisting}[language=Python, caption={ErrorMeasures}, label={ErrorMeasures}]
from pandas import read_excel
from matplotlib import pyplot
AustralianBeer  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [1],
                             header=0, squeeze=True, dtype=float)
NaiveF1  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [2],
                      header=0, squeeze=True, dtype=float)
NaiveF2 = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols=[3],
                     header=0, squeeze=True, dtype=float)

# Joint plot of original data and NF1 forecasts
AustralianBeer.plot(legend=True)
NaiveF1.plot(legend=True)
pyplot.show()

# Joint plot of original data and NF2 forecasts
AustralianBeer.plot(legend=True)
NaiveF2.plot(legend=True)
pyplot.show()

# Evaluating the errors from both NF1 and NF2 methods
Error1 = AustralianBeer - NaiveF1
Error2 = AustralianBeer - NaiveF2
ME1 = sum(Error1)* 1.0/len(NaiveF1)
ME2 = sum(Error2)* 1.0/len(NaiveF2)
MAE1=sum(abs(Error1))*1.0/len(NaiveF1)
MAE2=sum(abs(Error2))*1.0/len(NaiveF2)
MSE1=sum(Error1**2)*1.0/len(NaiveF1)
MSE2=sum(Error2**2)*1.0/len(NaiveF2)

PercentageError1=(Error1/AustralianBeer)*100
PercentageError2=(Error2/AustralianBeer)*100
MPE1 = sum(PercentageError1)* 1.0/len(NaiveF1)
MPE2 = sum(PercentageError2)* 1.0/len(NaiveF2)
MAE1=sum(abs(PercentageError1))*1.0/len(NaiveF1)
MAE2=sum(abs(PercentageError2))*1.0/len(NaiveF2)


#Printing a summary of the errors in a tabular form
print('Summary of errors resulting from NF1 & NF2:')
import pandas as pd
cars = {'Errors': ['ME','MAE','MSE','MPE', 'MAPE'],
        'NF1': [ME1, MAE1, MSE1, MPE1, MAE1],
        'NF2': [ME2, MAE2, MSE2, MPE2, MAE2]
        }
AllErrors = pd.DataFrame(cars, columns = ['Errors', 'NF1', 'NF2'])
print(AllErrors)
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={ACFErrors}, label={ACFErrors}]
from pandas import read_excel
from matplotlib import pyplot
AustralianBeer  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [1],
                             header=0, squeeze=True, dtype=float)
NaiveF1  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [2],
                      header=0, squeeze=True, dtype=float)
NaiveF2 = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols=[3],
                     header=0, squeeze=True, dtype=float)

# Plot for the original data set
AustralianBeer.plot(label='Original data', legend=True)
pyplot.show()

# Evaluating the errors from both NF1 and NF2 methods
Error1 = AustralianBeer - NaiveF1
Error2 = AustralianBeer - NaiveF2

# Plot of the error time series
Error1.plot(label='NF1 error plot', legend=True)
Error2.plot(label='NF2 error plot', legend=True)
pyplot.show()

# Creating an autocorrelation plot
from pandas.plotting import autocorrelation_plot
autocorrelation_plot(Error1)
autocorrelation_plot(Error2)
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={ConfidenceInterval}, label={ConfidenceInterval}]
from pandas import read_excel
from matplotlib import pyplot
from numpy import sqrt
AustralianBeer  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [1],
                             header=0, squeeze=True, dtype=float)
NaiveF1  = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols = [2],
                      header=0, squeeze=True, dtype=float)
NaiveF2 = read_excel('BeerErrorsData.xls', sheet_name='NF1NF2', usecols=[3],
                     header=0, squeeze=True, dtype=float)



# Evaluating the errors from both NF1 and NF2 methods
Error1 = AustralianBeer - NaiveF1
Error2 = AustralianBeer - NaiveF2
MSE1=sum(Error1**2)*1.0/len(NaiveF1)
MSE2=sum(Error2**2)*1.0/len(NaiveF2)

LowerForecast1 = NaiveF1 - 1.645*sqrt(MSE1)
UpperForecast1 = NaiveF1 + 1.645*sqrt(MSE1)

LowerForecast2 = NaiveF2 - 1.645*sqrt(MSE2)
UpperForecast2 = NaiveF2 + 1.645*sqrt(MSE2)

# Joint plot of original data and NF1 forecasts
AustralianBeer.plot(label='Original data')
NaiveF1.plot(label='NF1 forecast')
LowerForecast1.plot(label='NF1 lower bound')
UpperForecast1.plot(label='NF1 upper bound')
pyplot.legend()
pyplot.show()

# Joint plot of original data and NF2 forecasts
AustralianBeer.plot(label='Original data')
NaiveF2.plot(label='NF2 forecast')
LowerForecast2.plot(label='NF2 lower bound')
UpperForecast2.plot(label='NF2 upper bound')
pyplot.legend()
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={SimpleExpSmoothing}, label={SimpleExpSmoothing}]
from pandas import read_excel
from statsmodels.tsa.api import SimpleExpSmoothing
from matplotlib import pyplot
series = read_excel('ShampooSales.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)

# Simple Exponential Smoothing #

## SES model 1: alpha = 0.1
fit1 = SimpleExpSmoothing(series).fit(smoothing_level=0.1,optimized=False)
fcast1 = fit1.forecast(10).rename(r'$\alpha=0.1$')
# Plot of fitted values and forecast of next 10 values, respectively
fit1.fittedvalues.plot(color='blue')
fcast1.plot(color='blue', legend=True)

## SES model 2: alpha = 0.7
fit2 = SimpleExpSmoothing(series).fit(smoothing_level=0.7,optimized=False)
fcast2 = fit2.forecast(10).rename(r'$\alpha=0.7$')
# Plot of fitted values and forecast of next 10 values, respectively
fcast2.plot(color='red', legend=True)
fit2.fittedvalues.plot(color='red')

## SES model 3: alpha automatically selected by the built-in optimization software
fit3 = SimpleExpSmoothing(series).fit()
fcast3 = fit3.forecast(10).rename(r'$\alpha=%s$'%fit3.model.params['smoothing_level'])
# Plot of fitted values and forecast of next 10 values, respectively
fcast3.plot(color='green', legend=True)
fit3.fittedvalues.plot(color='green')

# Plotting the original data together with the 3 forecast plots
series.plot(color='black', legend=True)
pyplot.show()

#Evaluating the errors
from sklearn.metrics import mean_squared_error
MSE1=mean_squared_error(fit1.fittedvalues, series)
MSE2=mean_squared_error(fit2.fittedvalues, series)
MSE3=mean_squared_error(fit3.fittedvalues, series)

print('Summary of errors resulting from SES models 1, 2 & 3:')
import pandas as pd
cars = {'Model': ['MSE'],
        'SES model 1': [MSE1],
        'SES model 2': [MSE2],
        'SES model 3': [MSE3]
        }
AllErrors = pd.DataFrame(cars, columns = ['Model', 'SES model 1', 'SES model 2', 'SES model 3'])
print(AllErrors)
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={Holt}, label={Holt}]
from pandas import read_excel
from statsmodels.tsa.api import Holt
from matplotlib import pyplot
series = read_excel('ShampooSales.xls', sheetname='Data', header=0,
              index_col=0, squeeze=True)

# Holt model 1: alpha = 0.8, beta=0.2
fit1 = Holt(series).fit(smoothing_level=0.8, smoothing_slope=0.2, optimized=False)
fcast1 = fit1.forecast(12).rename("Holt's linear trend")

fit2 = Holt(series, exponential=True).fit(smoothing_level=0.8, smoothing_slope=0.2, optimized=False)
fcast2 = fit2.forecast(12).rename("Exponential trend")

fit3 = Holt(series, damped=True).fit(smoothing_level=0.8, smoothing_slope=0.2)
fcast3 = fit3.forecast(12).rename("Additive damped trend")

fit4 = Holt(series).fit(optimized=True)
fcast4 = fit4.forecast(12).rename("Additive 2 damped trend")


fit1.fittedvalues.plot(color='blue')
fcast1.plot(color='blue', legend=True)

fit2.fittedvalues.plot(color='red')
fcast2.plot(color='red', legend=True)

fit3.fittedvalues.plot(color='green')
fcast3.plot(color='green', legend=True)

fcast4.plot(color='yellow', legend=True)

series.plot(color='black', legend=True)
pyplot.show()

#Evaluating the errors
from sklearn.metrics import mean_squared_error
MSE1=mean_squared_error(fit1.fittedvalues, series)
MSE2=mean_squared_error(fit2.fittedvalues, series)
MSE3=mean_squared_error(fit3.fittedvalues, series)

print('Summary of errors resulting from SES models 1, 2 & 3:')
import pandas as pd
cars = {'Model': ['MSE'],
        'LES model 1': [MSE1],
        'LES model 2': [MSE2],
        'LES model 3': [MSE3]
        }
AllErrors = pd.DataFrame(cars, columns = ['Model', 'LES model 1', 'LES model 2', 'LES model 3'])
print(AllErrors)
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={ExponentialSmoothing}, label={ExponentialSmoothing}]
from pandas import read_excel
import pandas as pd
from statsmodels.tsa.api import ExponentialSmoothing
from matplotlib import pyplot
series = read_excel('CementProduction.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)

# ===================================
# Holt-Winter method in different scenarios #
# ===================================
# ===================================
# Model 1: Holt-Winter method with additive trend and seasonality
# Here, alpha = 0.3, beta=0.5, gamma=0.7
# ===================================
fit1 = ExponentialSmoothing(series, seasonal_periods=12, trend='add', seasonal='add').fit(smoothing_level = 0.3, smoothing_slope=0.5,  smoothing_seasonal=0.7)
fit1.fittedvalues.plot(color='red')

# ===================================
# Model 2: Holt-Winter method with additive trend and multiplicative seasonality
# Here, alpha = 0.3, beta=0.5, gamma=0.7
# ===================================
fit2 = ExponentialSmoothing(series, seasonal_periods=12, trend='add', seasonal='mul').fit(smoothing_level = 0.3, smoothing_slope=0.5,  smoothing_seasonal=0.7)
fit2.fittedvalues.plot(color='blue')

# ===================================
# Model 3: Holt-Winter method with additive trend and seasonality
# Here, the parameters alpha, beta, and gamma are optimized
# ===================================
fit3 = ExponentialSmoothing(series, seasonal_periods=12, trend='add', seasonal='add').fit()
fit3.fittedvalues.plot(color='green')

# ===================================
# Model 4: Holt-Winter method with additive trend and multiplicative seasonality
# Here, the parameters alpha, beta, and gamma are optimized
# ===================================
fit4 = ExponentialSmoothing(series, seasonal_periods=12, trend='add', seasonal='mul').fit()
fit4.fittedvalues.plot(color='yellow')

print("Forecasting Cement Production with Holt-Winters method")
#=====================================
# Time and forecast plots
#=====================================
series.rename('Time plot of original series').plot(color='black', legend=True)
fit1.forecast(12).rename('Model 1: HW-additive seasonality').plot(color='red', legend=True)
fit2.forecast(12).rename('Model 2: HW-multiplicative seasonality').plot(color='blue', legend=True)
fit3.forecast(12).rename('Model 3: Opt HW-additive seasonality').plot(color='green', legend=True)
fit4.forecast(12).rename('Model 4: Opt HW-multiplicative seasonality').plot(color='yellow', legend=True)
pyplot.xlabel('Dates')
pyplot.ylabel('Values')
pyplot.title('HW method-based forecasts for cement production')
pyplot.show()


#====================================
# Evaluating the errors
#====================================
from sklearn.metrics import mean_squared_error
MSE1=mean_squared_error(fit1.fittedvalues, series)
MSE2=mean_squared_error(fit2.fittedvalues, series)
MSE3=mean_squared_error(fit3.fittedvalues, series)
MSE4=mean_squared_error(fit4.fittedvalues, series)

#=====================================
# Printing the paramters and errors for each scenario
#=====================================
results=pd.DataFrame(index=[r"alpha", r"beta", r"gamma", r"l0", "b0", "MSE"])
params = ['smoothing_level', 'smoothing_slope', 'smoothing_seasonal', 'initial_level', 'initial_slope']
results["HW model 1"] = [fit1.params[p] for p in params] + [MSE1]
results["HW model 2"] = [fit2.params[p] for p in params] + [MSE2]
results["HW model 3"] = [fit3.params[p] for p in params] + [MSE3]
results["HW model 4"] = [fit4.params[p] for p in params] + [MSE4]
print(results)

#=====================================
# Evaluating and plotting the residual series for each scenario
#=====================================
residuals1= fit1.fittedvalues - series
residuals2= fit2.fittedvalues - series
residuals3= fit3.fittedvalues - series
residuals4= fit4.fittedvalues - series
residuals1.rename('residual plot for model 1').plot(color='red', legend=True)
residuals2.rename('residual plot for model 2').plot(color='blue', legend=True)
residuals3.rename('residual plot for model 3').plot(color='green', legend=True)
residuals4.rename('residual plot for model 4').plot(color='yellow', legend=True)
pyplot.title('Residual plots for models 1-4')
pyplot.show()

#=====================================
# ACF plots of the residual series for each scenario
#=====================================
from statsmodels.graphics.tsaplots import plot_acf
plot_acf(residuals1, title='Residual ACF for model 1', lags=50)
plot_acf(residuals2, title='Residual ACF for model 2', lags=50)
plot_acf(residuals3, title='Residual ACF for model 3', lags=50)
plot_acf(residuals4, title='Residual ACF for model 4', lags=50)
pyplot.show()
\end{lstlisting}

\section{Codes on ARIMA methods}
\begin{lstlisting}[language=Python, caption={WhiteNoiseModel}, label={WhiteNoiseModel}]
from random import gauss
from random import seed
from pandas import Series
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
from matplotlib import pyplot

# seed random number generator
seed(1)
# create white noise series
series = [gauss(0.0, 1.0) for i in range(1000)]

# Once created, we can wrap the list in a Pandas Series for convenience.
series = Series(series)

# summary statistics of the artificially generated series
print('Statistics of the artificially generated series:')
print(series.describe())

# line plot of the artificially generated series
series.plot(title='Time plot of a white noise model')
pyplot.show()

# histogram plot of the artificially generated series
series.hist()

# ACF plot of an artificially generated white noise time series
plot_acf(series, title='ACF of a white noise model', lags=50)

# PACF plot of an artificially generated white noise time series
plot_pacf(series, title='PACF of a white noise model', lags=50)
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={AcfPacfPlotNonStationarity.py}, label={AcfPacfPlotDowJones.py}]
from pandas import read_excel
from matplotlib import pyplot
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
series = read_excel('DowJones.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)

# ACF plot on 50 time lags
plot_acf(series, title='ACF of Dow Jones time series', lags=50)

# PACF plot on 50 time lags
plot_pacf(series, title='PACF of Dow Jones time series', lags=50)
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={ADFtest.py}, label={ADFtest.py}]
from pandas import read_excel
import matplotlib.pyplot as plt
series = read_excel('BuildingMaterials.xls', sheetname='Data', header=0,
              index_col=0, parse_dates=True, squeeze=True)
series.plot(color='red')
plt.xlabel('Dates')
plt.ylabel('Production values')
plt.title('Building materials production from 1986 to 2008')
plt.show()
#------------------------
from pandas import read_excel
from matplotlib import pyplot
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
series = read_excel('BuildingMaterials.xls', sheet_name='Data', usecols = [1],
                             header=0, squeeze=True, dtype=float)
# ACF plot on 50 time lags
plot_acf(series, title='ACF of building materials time series', lags=50)

# PACF plot on 50 time lags
plot_pacf(series, title='PACF of building materials time series', lags=50)
pyplot.show()
#--------------------------------------------------
# calculate stationarity test of time series data
#from pandas import read_csv
from statsmodels.tsa.stattools import adfuller
#series = read_csv('airline-passengers.csv', header=0, index_col=0, parse_dates=True,squeeze=True)
X = series.values
result = adfuller(X)
print('ADF Statistic: %f' % result[0])
print('p-value: %f' % result[1])
print('Critical Values:')
for key, value in result[4].items():
    print('\t%s: %.3f' % (key, value))
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={AcfPacfAR1model.py}, label={AcfPacfAR1model.py}]
from pandas import read_excel
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
from matplotlib import pyplot

series = read_excel('DataAR1model.xls', sheet_name='ARdata', header=0, index_col=0, squeeze=True)

# Time, ACF, and PACF plots for original data
pyplot.plot(series)
pyplot.title('Time plot AR1 data')
plot_acf(series, title='ACF plot of AR1 data', lags=20)
plot_pacf(series, title='PACF plot of AR1 data', lags=20)
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={AcfPacfMA1model.py}, label={AcfPacfMA1model.py}]
from pandas import read_excel
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
from matplotlib import pyplot

series = read_excel('DataMA1model.xls', sheet_name='MAdata', usecols = [1],
                    header=0, squeeze=True)

# Time, ACF, and PACF plots for original data
pyplot.plot(series)
pyplot.title('Time plot MA1 data')
plot_acf(series, title='ACF plot of MA1 data', lags=20)
plot_pacf(series, title='PACF plot of MA1 data', lags=20)
pyplot.show()
\end{lstlisting}


\begin{lstlisting}[language=Python, caption={AutomaticOrderARIMA.py}, label={AutomaticOrderARIMA.py}]
#===================================================
#Code for identifying the parameters with smallest AIC
#===================================================
from pandas import read_excel
from statsmodels.tsa.arima_model import ARIMA
import warnings
import itertools

series = read_excel('BuildingMaterials.xls', sheet_name='Data', header=0, index_col=0, parse_dates=True, squeeze=True)

#define the p, d and q parameters to take any value between 0 and 2
p = d = q = range(0, 3)

#generate all different combinations of p, q and q triplets
pdq = list(itertools.product(p, d, q))

#indentification of best model from different combinations of pdq
warnings.filterwarnings("ignore") # specify to ignore warning messages
best_score, best_param = float("inf"), None
for param in pdq:
        try:
            mod = ARIMA(series, param)
            results = mod.fit()
            if results.aic < best_score:
                best_score, best_param = results.aic, param
            print('ARIMA{} - AIC:{}'.format(param, results.aic))
        except:
            continue
print('The best model is ARIMA{} - AIC:{}'.format(best_param, best_score))
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={ARIMA.py}, label={ARIMA.py}]
from pandas import read_excel
import matplotlib.pyplot as plt
from statsmodels.tsa.arima_model import ARIMA

series = read_excel('BuildingMaterials.xls', sheet_name='Data', header=0,
                index_col=0, parse_dates=True, squeeze=True)

#ARIMA(1,1,2) model
model = ARIMA(series, order=(1,1,2))

# generates ARIMA Model Results table
model_fit = model.fit(disp=0)
fitted = model.fit(disp=1)
print(model_fit.summary())

# Actual vs Fitted
model_fit.plot_predict(dynamic=False)
plt.show()

# Forecast
fc, se, conf = fitted.forecast(15, alpha=0.005)  # 95% conf

pred_ci = pred_uc.conf_int()
# plotting forecasts ahead
ax = series.plot(label='Original data')
pred_uc.predicted_mean.plot(ax=ax, label='Forecast values', title='Forecast plot with confidence interval')
ax.fill_between(pred_ci.index,
                pred_ci.iloc[:, 0],
                pred_ci.iloc[:, 1], color='k', alpha=.25)
plt.legend()
plt.show()
#====================================================================

#====================================================================
# MSE evaluation
y_forecasted = pred.predicted_mean
y_truth = series['2000-01-01':]
# Compute the mean square error
MSE = ((y_forecasted - y_truth) ** 2).mean()
print('MSE of the forecasts is {}'.format(round(MSE, 2)))
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={FirstSeasonalDifference.py}, label={FirstSeasonalDifference.py}]
## removing seasonality from time series using seasonal differencing
from pandas import read_excel
from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
from matplotlib import pyplot

series = read_excel('Electricity.xls', sheet_name='ELEC', header=0, index_col=0, parse_dates=True, squeeze=True)

# Time, ACF, and PACF plots for original data
pyplot.plot(series)
pyplot.title('Time plot original data')
plot_acf(series, title='ACF plot of original data', lags=50)
plot_pacf(series, title='PACF plot of original data', lags=50)
pyplot.show()

#  Seaonal difference
X = series.values
SeasDiff = list()
for i in range(12, len(X)):
	value = X[i] - X[i - 12]
	SeasDiff.append(value)

# Time, ACF, and PACF plots for the seasonally differenced series
pyplot.plot(SeasDiff)
pyplot.title('Time plot seasonally differenced series')
plot_acf(SeasDiff, title='ACF plot of seasonally differenced series', lags=50)
plot_pacf(SeasDiff, title='PACF plot of seasonally differenced series', lags=50)
pyplot.show()

### Seasonal + First difference
Y = SeasDiff
SeasFirstDiff = list()
for i in range(1, len(Y)):
	value = Y[i] - Y[i - 1]
	SeasFirstDiff.append(value)
pyplot.plot(SeasFirstDiff)
pyplot.title('Time plot seasonally + first differenced series')
plot_acf(SeasFirstDiff, title='ACF plot of seasonally + first differenced series', lags=50)
plot_pacf(SeasFirstDiff, title='PACF plot of seasonally + first differenced series', lags=50)
pyplot.show()
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={AutomaticOrderSARIMAX.py}, label={AutomaticOrderSARIMAX.py}]
#===================================================
#Code for identifying the parameters with smallest AIC
#===================================================
from pandas import read_excel
import matplotlib.pyplot as plt
import statsmodels.api as sm
import warnings
import itertools
plt.style.use('fivethirtyeight')

series = read_excel('BuildingMaterials.xls', sheet_name='Data', header=0, index_col=0, parse_dates=True, squeeze=True)

#Define the p, d and q parameters to take any value between 0 and 1
p = d = q = range(0, 2)

# Generate all different combinations of p, q and q triplets
pdq = list(itertools.product(p, d, q))

# Generate all different combinations of seasonal p, q and q triplets (i.e., P, D, Q)
seasonal_pdq = [(x[0], x[1], x[2], 12) for x in list(itertools.product(p, d, q))]

# Indentification of best model from different combinations of pdq and seasonal_pdq
warnings.filterwarnings("ignore") # specify to ignore warning messages
best_score, best_param, best_paramSeasonal = float("inf"), None, None
for param in pdq:
    for param_seasonal in seasonal_pdq:
        try:
            mod = sm.tsa.statespace.SARIMAX(series, order=param, seasonal_order=param_seasonal, enforce_invertibility=False)
            results = mod.fit()
            if results.aic < best_score:
                best_score, best_param, best_paramSeasonal = results.aic, param, param_seasonal
            print('ARIMA{}x{} - AIC:{}'.format(param, param_seasonal, results.aic))
        except:
            continue
print('The best model is ARIMA{}x{} - AIC:{}'.format(best_param, best_paramSeasonal, best_score))
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={SARIMAX.py}, label={SARIMAX.py}]
from pandas import read_excel
import pandas as pd
import matplotlib.pyplot as plt
import statsmodels.api as sm
plt.style.use('fivethirtyeight')

#==================================================================
#Loading the data set
df = read_excel('BuildingMaterials.xls', sheet_name='Data', header=0,
                index_col=0, parse_dates=True, squeeze=True)
#==================================================================

#==================================================================
#Fitting the ARIMA model and printing related statistics
# ARIMA(0, 1, 1)(0,1,1)12 in this case;
#this one is based on MA1 model template
mod = sm.tsa.statespace.SARIMAX(df, order=(1,1,1), seasonal_order=(0,1,1,12))
results = mod.fit(disp=False)
print(results.summary())
#==================================================================

#GRAPH BLOCK1======================================================
#Printing the graphical statistics of model (correlogram = ACF plot)
results.plot_diagnostics(figsize=(15, 12))
plt.show()
#==================================================================

#GRAPH BLOCK2======================================================
# printing the part of forecasts fitted to original data (for accuracy evaluation)
# the start date has to be provided; hence should be a time within the original time series;
# in this case, it is to start on 01 January 2000
pred = results.get_prediction(start=pd.to_datetime('2000-01-01'), dynamic=False)
pred_ci = pred.conf_int()

# printing one-step ahead forecasts together with the original data set;
# hence, the starting point (year) of the data set is required
# in order to build the plot of original series
ax = df['1986':].plot(label='Original data')
pred.predicted_mean.plot(ax=ax, label='One-step ahead Forecast', alpha=.7)
ax.fill_between(pred_ci.index,
                pred_ci.iloc[:, 0],
                pred_ci.iloc[:, 1], color='k', alpha=.2)
plt.legend()
plt.show()
#===================================================================

#GRAPH BLOCK3=======================================================
# Get forecast 20 steps ahead in future
pred_uc = results.get_forecast(steps=20)
# Get confidence intervals of forecasts
pred_ci = pred_uc.conf_int()
# plotting forecasts ahead
ax = df.plot(label='Original data')
pred_uc.predicted_mean.plot(ax=ax, label='Forecast values', title='Forecast plot with confidence interval')
ax.fill_between(pred_ci.index,
                pred_ci.iloc[:, 0],
                pred_ci.iloc[:, 1], color='k', alpha=.25)
plt.legend()
plt.show()
#====================================================================

#====================================================================
# MSE evaluation
y_forecasted = pred.predicted_mean
y_truth = df['2000-01-01':]
# Compute the mean square error
MSE = ((y_forecasted - y_truth) ** 2).mean()
print('MSE of the forecasts is {}'.format(round(MSE, 2)))
#====================================================================
\end{lstlisting}

%\begin{lstlisting}[language=Python, caption=Demo 4.3 (ACF + PACF of Dow Jones time series)]
%from pandas import read_excel
%from matplotlib import pyplot
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%series = read_excel('DowJones.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%# ACF plot on 50 time lags
%plot_acf(series, title='ACF of Dow Jones time series', lags=50)
%
%# PACF plot on 50 time lags
%plot_pacf(series, title='PACF of Dow Jones time series', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.4 (Time/ACF/PACF plot Dow Jones 1st difference)]
%## detrend a time series using differencing
%from pandas import read_excel
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%from matplotlib import pyplot
%
%series = read_excel('DowJones.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%X = series.values
%diff = list()
%for i in range(1, len(X)):
%	value = X[i] - X[i - 1]
%	diff.append(value)
%pyplot.plot(diff)
%pyplot.title('Time plot Dow Jones 1st difference')
%
%# ACF plot of time series
%plot_acf(diff, title='ACF of Dow Jones 1st difference', lags=50)
%
%# PACF plot of time series
%plot_pacf(diff, title='PACF of Dow Jones 1st difference', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.5 (Seasonal differencing)]
%from pandas import read_excel
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%from matplotlib import pyplot
%
%series = read_excel('Electricity.xls', sheet_name='ELEC', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%# Time, ACF, and PACF plots for original data
%pyplot.plot(series)
%pyplot.title('Time plot original data')
%plot_acf(series, title='ACF plot of original data', lags=50)
%plot_pacf(series, title='PACF plot of original data', lags=50)
%pyplot.show()
%
%#  Seaonal difference
%X = series.values
%SeasDiff = list()
%for i in range(12, len(X)):
%	value = X[i] - X[i - 12]
%	SeasDiff.append(value)
%
%# Time, ACF, and PACF plots for the seasonally differenced series
%pyplot.plot(SeasDiff)
%pyplot.title('Time plot seasonally differenced series')
%plot_acf(SeasDiff, title='ACF plot of seasonally differenced series', lags=50)
%plot_pacf(SeasDiff, title='PACF plot of seasonally differenced series', lags=50)
%pyplot.show()
%
%### Seasonal + First difference
%Y = SeasDiff
%SeasFirstDiff = list()
%for i in range(1, len(Y)):
%	value = Y[i] - Y[i - 1]
%	SeasFirstDiff.append(value)
%pyplot.plot(SeasFirstDiff)
%pyplot.title('Time plot seasonally + first differenced series')
%plot_acf(SeasFirstDiff, title='ACF plot of seasonally + first differenced series', lags=50)
%plot_pacf(SeasFirstDiff, title='PACF plot of seasonally + first differenced series', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%
%
%
%
%\begin{lstlisting}[language=Python, caption=Demo 4.8--1 (Building an ARIMA model)]
%from pandas import read_excel
%from matplotlib import pyplot
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%series = read_excel('PrintingWriting.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%# ACF plot on 50 time lags
%plot_acf(series, title='ACF printing & writing paper sales', lags=50)
%
%# PACF plot on 50 time lags
%plot_pacf(series, title='PACF printing & writing paper sales', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.8--2 (Building an ARIMA model)]
%## removing seasonality from time series using seasonal differencing
%from pandas import read_excel
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%from matplotlib import pyplot
%
%series = read_excel('PrintingWriting.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%## Time, ACF, and PACF plots for original data
%#pyplot.plot(series)
%#pyplot.title('Time plot original data')
%#plot_acf(series, title='ACF plot of original data', lags=50)
%#plot_pacf(series, title='PACF plot of original data', lags=50)
%#pyplot.show()
%
%#  Seaonal difference
%X = series.values
%SeasDiff = list()
%for i in range(12, len(X)):
%	value = X[i] - X[i - 12]
%	SeasDiff.append(value)
%
%# Time, ACF, and PACF plots for the seasonally differenced series
%pyplot.plot(SeasDiff)
%pyplot.title('Time plot seasonally differenced series')
%plot_acf(SeasDiff, title='ACF plot of seasonally differenced series', lags=50)
%plot_pacf(SeasDiff, title='PACF plot of seasonally differenced series', lags=50)
%pyplot.show()
%
%# Seasonal + First difference
%Y = SeasDiff
%SeasFirstDiff = list()
%for i in range(1, len(Y)):
%	value = Y[i] - Y[i - 1]
%	SeasFirstDiff.append(value)
%pyplot.plot(SeasFirstDiff)
%pyplot.title('Time plot seasonally + first differenced series')
%plot_acf(SeasFirstDiff, title='ACF plot of seasonally + first differenced series', lags=50)
%plot_pacf(SeasFirstDiff, title='PACF plot of seasonally + first differenced series', lags=50)
%pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.8--3 (Building an ARIMA model)]
%## removing seasonality from time series using seasonal differencing
%from pandas import read_excel
%from statsmodels.graphics.tsaplots import plot_acf, plot_pacf
%from matplotlib import pyplot
%
%series = read_excel('PrintingWriting.xls', sheet_name='Data2', header=0, index_col=0, parse_dates=True, squeeze=True)
%
%## Time, ACF, and PACF plots for original data
%#pyplot.plot(series)
%#pyplot.title('Time plot original data')
%#plot_acf(series, title='ACF plot of original data', lags=50)
%#plot_pacf(series, title='PACF plot of original data', lags=50)
%#pyplot.show()
%
%#  Seaonal difference
%X = series.values
%SeasDiff = list()
%for i in range(12, len(X)):
%	value = X[i] - X[i - 12]
%	SeasDiff.append(value)
%
%# Time, ACF, and PACF plots for the seasonally differenced series
%pyplot.plot(SeasDiff)
%pyplot.title('Time plot seasonally differenced series')
%plot_acf(SeasDiff, title='ACF plot of seasonally differenced series', lags=50)
%plot_pacf(SeasDiff, title='PACF plot of seasonally differenced series', lags=50)
%pyplot.show()
%
%#### Seasonal + First difference
%#Y = SeasDiff
%#SeasFirstDiff = list()
%#for i in range(1, len(Y)):
%#	value = Y[i] - Y[i - 1]
%#	SeasFirstDiff.append(value)
%#pyplot.plot(SeasFirstDiff)
%#pyplot.title('Time plot seasonally + first differenced series')
%#plot_acf(SeasFirstDiff, title='ACF plot of seasonally + first differenced series', lags=50)
%#plot_pacf(SeasFirstDiff, title='PACF plot of seasonally + first differenced series', lags=50)
%#pyplot.show()
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 4.8--4 (Building an ARIMA model)]
%from pandas import read_excel
%import pandas as pd
%import matplotlib.pyplot as plt
%import statsmodels.api as sm
%plt.style.use('fivethirtyeight')
%
%###############################
%df = read_excel('PrintingWriting.xls', sheet_name='Data2', header=0,
%               index_col=0, parse_dates=True, squeeze=True)
%
%# ARIMA model with (p, d, q)=(1, 1, 1)
%#mod = sm.tsa.statespace.SARIMAX(df, trend='c', order=(1,1,1))
%mod = sm.tsa.statespace.SARIMAX(df, order=(1,1,1),
%                                seasonal_order=(1,1,1,12))
%results = mod.fit(disp=False)
%print(results.summary())
%
%# graphical statistics of model (correlogram = ACF plot)
%results.plot_diagnostics(figsize=(15, 12))
%plt.show()
%
%#============================================
%# this code requires the fitted forecasts (for accuracy evaluation) to start 01 Jan 1979.
%pred = results.get_prediction(start=pd.to_datetime('1972-01-01'), dynamic=False)
%pred_ci = pred.conf_int()
%
%print(pred_ci)
%
%# this code requires the whole plot to start in 1956 (start year of data)
%ax = df['1969':].plot(label='Original data')
%pred.predicted_mean.plot(ax=ax, label='One-step ahead Forecast', alpha=.7)
%
%ax.fill_between(pred_ci.index,
%                pred_ci.iloc[:, 0],
%                pred_ci.iloc[:, 1], color='k', alpha=.2)
%plt.legend()
%plt.show()
%#=============================================
%# MSE evaluation
%y_forecasted = pred.predicted_mean
%y_truth = df['1965-01-01':]
%# Compute the mean square error
%mse = ((y_forecasted - y_truth) ** 2).mean()
%print('MSE of the forecasts is {}'.format(round(mse, 2)))
%
%#=============================================
%# get forecast 20 steps ahead in future
%pred_uc = results.get_forecast(steps=20)
%# Get confidence intervals of forecasts
%pred_ci = pred_uc.conf_int()
%
%# plotting forecasts ahead
%ax = df.plot(label='Original data')
%pred_uc.predicted_mean.plot(ax=ax, label='Forecast values', title='Forecast plot with confidence interval')
%ax.fill_between(pred_ci.index,
%                pred_ci.iloc[:, 0],
%                pred_ci.iloc[:, 1], color='k', alpha=.25)
%plt.legend()
%plt.show()
%#----------------------------------------------
%\end{lstlisting}

\section{Codes on the regression analysis and application to forecasting}

%\begin{lstlisting}[language=Python, caption={RegressionTimePlot.py}, label={RegressionTimePlot.py}]
%from pandas import read_excel
%import matplotlib.pyplot as plt
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%DEOM.plot()
%plt.xlabel('time')
%plt.ylabel('Difference end of month balance')
%plt.title('DEOM')
%plt.show()
%
%AAA.plot()
%plt.xlabel('time')
%plt.ylabel('Composite AAA Bond rates')
%plt.title('AAA')
%plt.show()
%
%Tto4.plot()
%plt.xlabel('time')
%plt.ylabel('US Govt 3-4 year Bond rates')
%plt.title('3to4')
%plt.show()
%
%D3to4.plot()
%plt.xlabel('time')
%plt.ylabel('Difference US Govt 3-4 year Bond rates')
%plt.title('D3to4')
%plt.show()
%\end{lstlisting}



\begin{lstlisting}[language=Python, caption={RegressionAnalysis.py}, label={Regression.py}]
from pandas import read_excel
from statsmodels.formula.api import ols
series = read_excel('Bank.xls', sheet_name='Data2', header=0,
                     squeeze=True, dtype=float)

#reading the basic variables
DEOM = series.DEOM
AAA = series.AAA
Tto4 = series.Tto4
D3to4 = series.D3to4

#Regression model(s)
formula = 'DEOM ~ AAA + Tto4 + D3to4'

#Ordinary Least Squares (OLS)
results = ols(formula, data=series).fit()
print(results.summary())

# Here the main table is the first one,
# where the main statistics are the R-squared (line 1)
# and the P-value; i.e., Prob (F-statistic)
\end{lstlisting}


%\begin{lstlisting}[language=Python, caption=Demo 3.3 (Individual significance analysis)]
%from pandas import read_excel
%from statsmodels.formula.api import ols
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%#Regression model(s)
%formula = 'DEOM ~ AAA + Tto4 + D3to4'
%
%#Ordinary Least Squares (OLS)
%results = ols(formula, data=series).fit()
%print(results.summary())
%
%# Here the main table is the second one,
%# where all the statistics of the individual variables
%# are given.
%\end{lstlisting}
%
%
%\begin{lstlisting}[language=Python, caption=Demo 3.4 (Statistics for model with indicator variables)]
%from pandas import read_excel
%from statsmodels.formula.api import ols
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%#reading the indicator variables
%D1=series.D1
%D2=series.D2
%D3=series.D3
%D4=series.D4
%D5=series.D5
%D6=series.D6
%D7=series.D7
%D8=series.D8
%D9=series.D9
%D10=series.D10
%D11=series.D11
%
%#Regression model(s)
%formula = 'DEOM ~ AAA + Tto4 + D3to4 + D1 + D2 + D3+D4+D5+D6+D7+D8+D9+D10+D11'
%
%
%#Ordinary Least Squares (OLS)
%results = ols(formula, data=series).fit()
%print(results.summary())
%
%# the two tables show the changes in the overall and
%# individual significance of the model when
%# the indicator variables (Di, i=1, ..., 11) are added
%# Pay attention to the changes in the key statistics
%\end{lstlisting}
%
%\begin{lstlisting}[language=Python, caption=Demo 3.5 (Statistics for model with indicator + time variables)]
%from pandas import read_excel
%from statsmodels.formula.api import ols
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%#reading the indicator variables
%D1=series.D1
%D2=series.D2
%D3=series.D3
%D4=series.D4
%D5=series.D5
%D6=series.D6
%D7=series.D7
%D8=series.D8
%D9=series.D9
%D10=series.D10
%D11=series.D11
%
%#reading the time variable
%time=series.time
%
%#Regression model(s)
%formula = 'DEOM ~ AAA + Tto4 + D3to4 + D1 + D2 + D3+D4+D5+D6+D7+D8+D9+D10+D11+time'
%
%#Ordinary Least Squares (OLS)
%results = ols(formula, data=series).fit()
%print(results.summary())
%
%# the difference with what is done
%# in StatsWithIndicatorsBank.py is the addition of time
%# So the same statistics remain important to see the changes
%\end{lstlisting}
%
%
%\begin{lstlisting}[language=Python, caption=Demo 3.6 (Statistics comparision)]
%from pandas import read_excel
%from statsmodels.formula.api import ols
%series = read_excel('Bank.xls', sheet_name='Data2', header=0,
%                     squeeze=True, dtype=float)
%
%#reading the basic variables
%DEOM = series.DEOM
%AAA = series.AAA
%Tto4 = series.Tto4
%D3to4 = series.D3to4
%
%#reading the indicator variables
%D1=series.D1
%D2=series.D2
%D3=series.D3
%D4=series.D4
%D5=series.D5
%D6=series.D6
%D7=series.D7
%D8=series.D8
%D9=series.D9
%D10=series.D10
%D11=series.D11
%
%#reading the time variable
%time=series.time
%
%#Regression model(s)
%formula1 = 'DEOM ~ AAA + Tto4 + D3to4'
%formula2 = 'DEOM ~ AAA + Tto4 + D3to4 + D1 + D2 + D3+D4+D5+D6+D7+D8+D9+D10+D11'
%formula3 = 'DEOM ~ AAA + Tto4 + D3to4 + D1 + D2 + D3+D4+D5+D6+D7+D8+D9+D10+D11+time'
%
%#Ordinary Least Squares (OLS)
%results1 = ols(formula1, data=series).fit()
%results2 = ols(formula2, data=series).fit()
%results3 = ols(formula3, data=series).fit()
%print(results1.summary())
%print(results2.summary())
%print(results3.summary())
%
%# the results from IndividualSignificance.py,
%# StatsWithIndicatorsBank.py,
%# and StatsWithIndicatorsTimeBank.py are summarised
%# for easy comparison of the key statistics
%\end{lstlisting}


\begin{lstlisting}[language=Python, caption={RegressionForecast.py}, label={RegressionForecast.py}]
from pandas import read_excel
from statsmodels.tsa.api import Holt
#from matplotlib import pyplot
import matplotlib.pyplot as plt
import numpy as np
from statsmodels.formula.api import ols
series = read_excel('Bank.xls', sheet_name='Data2', header=0,
                     squeeze=True, dtype=float)

# Reading the basic variables
DEOM = series.DEOM
AAA = series.AAA
Tto4 = series.Tto4
D3to4 = series.D3to4

# Forecasting for AAA using Holt's linear method
fit1 = Holt(AAA).fit(optimized=True)
fcast1 = fit1.forecast(6).rename("Additive 2 damped trend")
fit1.fittedvalues.plot(color='red')
fcast1.plot(color='red', legend=True)
AAA.plot(color='black', legend=True)
plt.title('Forecast of AAA with Holt linear method')
plt.show()

# Forecasting for Tto4 using Holt's linear method
fit2 = Holt(Tto4).fit(optimized=True)
fcast2 = fit2.forecast(6).rename("Additive 2 damped trend")
fit2.fittedvalues.plot(color='red')
fcast2.plot(color='red', legend=True)
Tto4.plot(color='black', legend=True)
plt.title('Forecast of 3to4 with Holt linear method')
plt.show()

# Forecasting for D3to4 using Holt's linear method
fit3 = Holt(D3to4).fit(smoothing_level=0.8, smoothing_slope=0.2, optimized=False)
#fit3 = Holt(D3to4).fit(optimized=True)
fcast3 = fit3.forecast(6).rename("Additive 2 damped trend")
fit3.fittedvalues.plot(color='red')
fcast3.plot(color='red', legend=True)
D3to4.plot(color='black', legend=True)
plt.title('Forecast of D3to4 with Holt linear method')
plt.show()

# Building the regression based forecast for main variable, DEOM
# Regression model(s)
formula = 'DEOM ~ AAA + Tto4 + D3to4'

# ols generate statistics and the parameters b0, b1, etc., of the model
results = ols(formula, data=series).fit()
results.summary()
b0 = results.params.Intercept
b1 = results.params.AAA
b2 = results.params.Tto4
b3 = results.params.D3to4

# putting the fitted values of the forecasts of AAA, Tto4, and D3to4 in arrays
a1 = np.array(fit1.fittedvalues)
a2 = np.array(fit2.fittedvalues)
a3 = np.array(fit3.fittedvalues)

# Building the fitted part of the forecast of DEOM
F=a1
for i in range(53):
    F[i] = b0 + a1[i]*b1 + a2[i]*b2 + a3[i]*b3

# putting the values of the forecasts of AAA, Tto4, and D3to4 in arrays
v1=np.array(fcast1)
v2=np.array(fcast2)
v3=np.array(fcast3)

# Building the 6 values of the forecast ahead
E=v1
for i in range(6):
    E[i] = b0 + v1[i]*b1 + v2[i]*b2 + v3[i]*b3


# Joining the fitted values of the forecast and the points ahead
K=np.append(F, E)

# Reading the original DEOM time series for all the 59 periods
DEOMfull0 = read_excel('Bank.xls', sheet_name='Data4', header=0,
                     squeeze=True, dtype=float)

###########################
# Evaluating the MSE to generate the confidence interval
DEOMfull = DEOMfull0.DEOMfull
values=DEOMfull[0:53]
Error = values - F
MSE=sum(Error**2)*1.0/len(F)

## Lower and upper bounds of forecasts for z=1.282; see equation (2.2) in Chap 2.
#LowerE = E - 1.282*MSE
#UpperE = E + 1.282*MSE

LowerE = DEOMfull0.LowerE
UpperE = DEOMfull0.UpperE

print(LowerE)
###############################

# Plotting the graphs of K and DEOMfull with legends
from matplotlib.legend_handler import HandlerLine2D
line1, = plt.plot(K, color='red', label='Forecast values')
line2, = plt.plot(DEOMfull, color='black', label='Original data')
line3, = plt.plot(LowerE, color='blue', label='Lower forecast')
line4, = plt.plot(UpperE, color='orange', label='Upper forecast')
plt.legend(handler_map={line1: HandlerLine2D(numpoints=4)})
plt.title('DEOM regression forecast with confidence interval')
plt.show()

# Proceeding as as in other demos, forecasts
# can be generated for other scenarios; i.e., with different combinations of variables
\end{lstlisting}


==> structure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The Legrand Orange Book
% Structural Definitions File
% Version 2.0 (9/2/15)
%
% Original author:
% Mathias Legrand (legrand.mathias@gmail.com) with modifications by:
% Vel (vel@latextemplates.com)
% 
% This file has been downloaded from:
% http://www.LaTeXTemplates.com
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	VARIOUS REQUIRED PACKAGES AND CONFIGURATIONS
%----------------------------------------------------------------------------------------

\usepackage[top=3cm,bottom=3cm,left=3cm,right=3cm,headsep=10pt,a4paper]{geometry} % Page margins

\usepackage{graphicx} % Required for including pictures
\graphicspath{{Pictures/}} % Specifies the directory where pictures are stored

\usepackage{lipsum} % Inserts dummy text

\usepackage{tikz} % Required for drawing custom shapes

\usepackage[english]{babel} % English language/hyphenation

\usepackage{enumitem} % Customize lists
\setlist{nolistsep} % Reduce spacing between bullet points and numbered lists

\usepackage{booktabs} % Required for nicer horizontal rules in tables

\usepackage{xcolor} % Required for specifying colors by name
\definecolor{ocre}{RGB}{243,102,25} % Define the orange color used for highlighting throughout the book

%----------------------------------------------------------------------------------------
%	FONTS
%----------------------------------------------------------------------------------------

\usepackage{avant} % Use the Avantgarde font for headings
%\usepackage{times} % Use the Times font for headings
\usepackage{mathptmx} % Use the Adobe Times Roman as the default text font together with math symbols from the Sym­bol, Chancery and Com­puter Modern fonts

\usepackage{microtype} % Slightly tweak font spacing for aesthetics
\usepackage[utf8]{inputenc} % Required for including letters with accents
\usepackage[T1]{fontenc} % Use 8-bit encoding that has 256 glyphs

%----------------------------------------------------------------------------------------
%	BIBLIOGRAPHY AND INDEX
%----------------------------------------------------------------------------------------

\usepackage[style=alphabetic,citestyle=numeric,sorting=nyt,sortcites=true,autopunct=true,babel=hyphen,hyperref=true,abbreviate=false,backref=true,backend=biber]{biblatex}
\addbibresource{bibliography.bib} % BibTeX bibliography file
\defbibheading{bibempty}{}

\usepackage{calc} % For simpler calculation - used for spacing the index letter headings correctly
\usepackage{makeidx} % Required to make an index
\makeindex % Tells LaTeX to create the files required for indexing

%----------------------------------------------------------------------------------------
%	MAIN TABLE OF CONTENTS
%----------------------------------------------------------------------------------------

\usepackage{titletoc} % Required for manipulating the table of contents

\contentsmargin{0cm} % Removes the default margin

% Part text styling
\titlecontents{part}[0cm]
{\addvspace{20pt}\centering\large\bfseries}
{}
{}
{}

% Chapter text styling
\titlecontents{chapter}[1.25cm] % Indentation
{\addvspace{12pt}\large\sffamily\bfseries} % Spacing and font options for chapters
{\color{ocre!60}\contentslabel[\Large\thecontentslabel]{1.25cm}\color{ocre}} % Chapter number
{\color{ocre}}  
{\color{ocre!60}\normalsize\;\titlerule*[.5pc]{.}\;\thecontentspage} % Page number

% Section text styling
\titlecontents{section}[1.25cm] % Indentation
{\addvspace{3pt}\sffamily\bfseries} % Spacing and font options for sections
{\contentslabel[\thecontentslabel]{1.25cm}} % Section number
{}
{\hfill\color{black}\thecontentspage} % Page number
[]

% Subsection text styling
\titlecontents{subsection}[1.25cm] % Indentation
{\addvspace{1pt}\sffamily\small} % Spacing and font options for subsections
{\contentslabel[\thecontentslabel]{1.25cm}} % Subsection number
{}
{\ \titlerule*[.5pc]{.}\;\thecontentspage} % Page number
[]

% List of figures
\titlecontents{figure}[0em]
{\addvspace{-5pt}\sffamily}
{\thecontentslabel\hspace*{1em}}
{}
{\ \titlerule*[.5pc]{.}\;\thecontentspage}
[]

% List of tables
\titlecontents{table}[0em]
{\addvspace{-5pt}\sffamily}
{\thecontentslabel\hspace*{1em}}
{}
{\ \titlerule*[.5pc]{.}\;\thecontentspage}
[]

%----------------------------------------------------------------------------------------
%	MINI TABLE OF CONTENTS IN PART HEADS
%----------------------------------------------------------------------------------------

% Chapter text styling
\titlecontents{lchapter}[0em] % Indenting
{\addvspace{15pt}\large\sffamily\bfseries} % Spacing and font options for chapters
{\color{ocre}\contentslabel[\Large\thecontentslabel]{1.25cm}\color{ocre}} % Chapter number
{}  
{\color{ocre}\normalsize\sffamily\bfseries\;\titlerule*[.5pc]{.}\;\thecontentspage} % Page number

% Section text styling
\titlecontents{lsection}[0em] % Indenting
{\sffamily\small} % Spacing and font options for sections
{\contentslabel[\thecontentslabel]{1.25cm}} % Section number
{}
{}

% Subsection text styling
\titlecontents{lsubsection}[.5em] % Indentation
{\normalfont\footnotesize\sffamily} % Font settings
{}
{}
{}

%----------------------------------------------------------------------------------------
%	PAGE HEADERS
%----------------------------------------------------------------------------------------

\usepackage{fancyhdr} % Required for header and footer configuration

\pagestyle{fancy}
\renewcommand{\chaptermark}[1]{\markboth{\sffamily\normalsize\bfseries\chaptername\ \thechapter.\ #1}{}} % Chapter text font settings
\renewcommand{\sectionmark}[1]{\markright{\sffamily\normalsize\thesection\hspace{5pt}#1}{}} % Section text font settings
\fancyhf{} \fancyhead[LE,RO]{\sffamily\normalsize\thepage} % Font setting for the page number in the header
\fancyhead[LO]{\rightmark} % Print the nearest section name on the left side of odd pages
\fancyhead[RE]{\leftmark} % Print the current chapter name on the right side of even pages
\renewcommand{\headrulewidth}{0.5pt} % Width of the rule under the header
\addtolength{\headheight}{2.5pt} % Increase the spacing around the header slightly
\renewcommand{\footrulewidth}{0pt} % Removes the rule in the footer
\fancypagestyle{plain}{\fancyhead{}\renewcommand{\headrulewidth}{0pt}} % Style for when a plain pagestyle is specified

% Removes the header from odd empty pages at the end of chapters
\makeatletter
\renewcommand{\cleardoublepage}{
\clearpage\ifodd\c@page\else
\hbox{}
\vspace*{\fill}
\thispagestyle{empty}
\newpage
\fi}

%----------------------------------------------------------------------------------------
%	THEOREM STYLES
%----------------------------------------------------------------------------------------

\usepackage{amsmath,amsfonts,amssymb,amsthm} % For math equations, theorems, symbols, etc

\newcommand{\intoo}[2]{\mathopen{]}#1\,;#2\mathclose{[}}
\newcommand{\ud}{\mathop{\mathrm{{}d}}\mathopen{}}
\newcommand{\intff}[2]{\mathopen{[}#1\,;#2\mathclose{]}}
\newtheorem{notation}{Notation}[chapter]

% Boxed/framed environments
\newtheoremstyle{ocrenumbox}% % Theorem style name
{0pt}% Space above
{0pt}% Space below
{\normalfont}% % Body font
{}% Indent amount
{\small\bf\sffamily\color{ocre}}% % Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\color{ocre}\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries\color{black}---\nobreakspace#3.}} % Optional theorem note
\renewcommand{\qedsymbol}{$\blacksquare$}% Optional qed square

\newtheoremstyle{blacknumex}% Theorem style name
{5pt}% Space above
{5pt}% Space below
{\normalfont}% Body font
{} % Indent amount
{\small\bf\sffamily}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily{\tiny\ensuremath{\blacksquare}}\nobreakspace\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries---\nobreakspace#3.}}% Optional theorem note

\newtheoremstyle{blacknumbox} % Theorem style name
{0pt}% Space above
{0pt}% Space below
{\normalfont}% Body font
{}% Indent amount
{\small\bf\sffamily}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries---\nobreakspace#3.}}% Optional theorem note

% Non-boxed/non-framed environments
\newtheoremstyle{ocrenum}% % Theorem style name
{5pt}% Space above
{5pt}% Space below
{\normalfont}% % Body font
{}% Indent amount
{\small\bf\sffamily\color{ocre}}% % Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\color{ocre}\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries\color{black}---\nobreakspace#3.}} % Optional theorem note
\renewcommand{\qedsymbol}{$\blacksquare$}% Optional qed square
\makeatother

% Defines the theorem text style for each type of theorem to one of the three styles above
\newcounter{dummy} 
\numberwithin{dummy}{section}
\theoremstyle{ocrenumbox}
\newtheorem{theoremeT}[dummy]{Theorem}
\newtheorem{problem}{Problem}[chapter]
\newtheorem{exerciseT}{Exercise}[chapter]
\theoremstyle{blacknumex}
\newtheorem{exampleT}{Example}[chapter]
\theoremstyle{blacknumbox}
\newtheorem{vocabulary}{Vocabulary}[chapter]
\newtheorem{definitionT}{Definition}[section]
\newtheorem{corollaryT}[dummy]{Corollary}
\theoremstyle{ocrenum}
\newtheorem{proposition}[dummy]{Proposition}

%----------------------------------------------------------------------------------------
%	DEFINITION OF COLORED BOXES
%----------------------------------------------------------------------------------------

\RequirePackage[framemethod=default]{mdframed} % Required for creating the theorem, definition, exercise and corollary boxes

% Theorem box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
backgroundcolor=black!5,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
innerbottommargin=5pt]{tBox}

% Exercise box	  
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
backgroundcolor=ocre!10,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
innerbottommargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt]{eBox}	

% Definition box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=0pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt,
innerbottommargin=0pt]{dBox}	

% Corollary box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
linecolor=gray,
backgroundcolor=black!5,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt,
innerbottommargin=5pt]{cBox}

% Creates an environment for each type of theorem and assigns it a theorem text style from the "Theorem Styles" section above and a colored box from above
\newenvironment{theorem}{\begin{tBox}\begin{theoremeT}}{\end{theoremeT}\end{tBox}}
\newenvironment{exercise}{\begin{eBox}\begin{exerciseT}}{\hfill{\color{ocre}\tiny\ensuremath{\blacksquare}}\end{exerciseT}\end{eBox}}				  
\newenvironment{definition}{\begin{dBox}\begin{definitionT}}{\end{definitionT}\end{dBox}}	
\newenvironment{example}{\begin{exampleT}}{\hfill{\tiny\ensuremath{\blacksquare}}\end{exampleT}}		
\newenvironment{corollary}{\begin{cBox}\begin{corollaryT}}{\end{corollaryT}\end{cBox}}	

%----------------------------------------------------------------------------------------
%	REMARK ENVIRONMENT
%----------------------------------------------------------------------------------------

\newenvironment{remark}{\par\vspace{10pt}\small % Vertical white space above the remark and smaller font size
\begin{list}{}{
\leftmargin=35pt % Indentation on the left
\rightmargin=25pt}\item\ignorespaces % Indentation on the right
\makebox[-2.5pt]{\begin{tikzpicture}[overlay]
\node[draw=ocre!60,line width=1pt,circle,fill=ocre!25,font=\sffamily\bfseries,inner sep=2pt,outer sep=0pt] at (-15pt,0pt){\textcolor{ocre}{R}};\end{tikzpicture}} % Orange R in a circle
\advance\baselineskip -1pt}{\end{list}\vskip5pt} % Tighter line spacing and white space after remark

%----------------------------------------------------------------------------------------
%	SECTION NUMBERING IN THE MARGIN
%----------------------------------------------------------------------------------------

\makeatletter
\renewcommand{\@seccntformat}[1]{\llap{\textcolor{ocre}{\csname the#1\endcsname}\hspace{1em}}}                    
\renewcommand{\section}{\@startsection{section}{1}{\z@}
{-4ex \@plus -1ex \@minus -.4ex}
{1ex \@plus.2ex }
{\normalfont\large\sffamily\bfseries}}
\renewcommand{\subsection}{\@startsection {subsection}{2}{\z@}
{-3ex \@plus -0.1ex \@minus -.4ex}
{0.5ex \@plus.2ex }
{\normalfont\sffamily\bfseries}}
\renewcommand{\subsubsection}{\@startsection {subsubsection}{3}{\z@}
{-2ex \@plus -0.1ex \@minus -.2ex}
{.2ex \@plus.2ex }
{\normalfont\small\sffamily\bfseries}}                        
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}
{-2ex \@plus-.2ex \@minus .2ex}
{.1ex}
{\normalfont\small\sffamily\bfseries}}

%----------------------------------------------------------------------------------------
%	PART HEADINGS
%----------------------------------------------------------------------------------------

% numbered part in the table of contents
\newcommand{\@mypartnumtocformat}[2]{%
\setlength\fboxsep{0pt}%
\noindent\colorbox{ocre!20}{\strut\parbox[c][.7cm]{\ecart}{\color{ocre!70}\Large\sffamily\bfseries\centering#1}}\hskip\esp\colorbox{ocre!40}{\strut\parbox[c][.7cm]{\linewidth-\ecart-\esp}{\Large\sffamily\centering#2}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% unnumbered part in the table of contents
\newcommand{\@myparttocformat}[1]{%
\setlength\fboxsep{0pt}%
\noindent\colorbox{ocre!40}{\strut\parbox[c][.7cm]{\linewidth}{\Large\sffamily\centering#1}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength\esp
\setlength\esp{4pt}
\newlength\ecart
\setlength\ecart{1.2cm-\esp}
\newcommand{\thepartimage}{}%
\newcommand{\partimage}[1]{\renewcommand{\thepartimage}{#1}}%
\def\@part[#1]#2{%
\ifnum \c@secnumdepth >-2\relax%
\refstepcounter{part}%
\addcontentsline{toc}{part}{\texorpdfstring{\protect\@mypartnumtocformat{\thepart}{#1}}{\partname~\thepart\ ---\ #1}}
\else%
\addcontentsline{toc}{part}{\texorpdfstring{\protect\@myparttocformat{#1}}{#1}}%
\fi%
\startcontents%
\markboth{}{}%
{\thispagestyle{empty}%
\begin{tikzpicture}[remember picture,overlay]%
\node at (current page.north west){\begin{tikzpicture}[remember picture,overlay]%	
\fill[ocre!20](0cm,0cm) rectangle (\paperwidth,-\paperheight);
\node[anchor=north] at (4cm,-3.25cm){\color{ocre!40}\fontsize{220}{100}\sffamily\bfseries\@Roman\c@part}; 
\node[anchor=south east] at (\paperwidth-1cm,-\paperheight+1cm){\parbox[t][][t]{8.5cm}{
\printcontents{l}{0}{\setcounter{tocdepth}{1}}%
}};
\node[anchor=north east] at (\paperwidth-1.5cm,-3.25cm){\parbox[t][][t]{15cm}{\strut\raggedleft\color{white}\fontsize{30}{30}\sffamily\bfseries#2}};
\end{tikzpicture}};
\end{tikzpicture}}%
\@endpart}
\def\@spart#1{%
\startcontents%
\phantomsection
{\thispagestyle{empty}%
\begin{tikzpicture}[remember picture,overlay]%
\node at (current page.north west){\begin{tikzpicture}[remember picture,overlay]%	
\fill[ocre!20](0cm,0cm) rectangle (\paperwidth,-\paperheight);
\node[anchor=north east] at (\paperwidth-1.5cm,-3.25cm){\parbox[t][][t]{15cm}{\strut\raggedleft\color{white}\fontsize{30}{30}\sffamily\bfseries#1}};
\end{tikzpicture}};
\end{tikzpicture}}
\addcontentsline{toc}{part}{\texorpdfstring{%
\setlength\fboxsep{0pt}%
\noindent\protect\colorbox{ocre!40}{\strut\protect\parbox[c][.7cm]{\linewidth}{\Large\sffamily\protect\centering #1\quad\mbox{}}}}{#1}}%
\@endpart}
\def\@endpart{\vfil\newpage
\if@twoside
\if@openright
\null
\thispagestyle{empty}%
\newpage
\fi
\fi
\if@tempswa
\twocolumn
\fi}

%----------------------------------------------------------------------------------------
%	CHAPTER HEADINGS
%----------------------------------------------------------------------------------------

% A switch to conditionally include a picture, implemented by  Christian Hupfer
\newif\ifusechapterimage
\usechapterimagetrue
\newcommand{\thechapterimage}{}%
\newcommand{\chapterimage}[1]{\ifusechapterimage\renewcommand{\thechapterimage}{#1}\fi}%
\def\@makechapterhead#1{%
{\parindent \z@ \raggedright \normalfont
\ifnum \c@secnumdepth >\m@ne
\if@mainmatter
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}\thechapter. #1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\else
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}#1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\fi\fi\par\vspace*{270\p@}}}

%-------------------------------------------

\def\@makeschapterhead#1{%
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}#1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\par\vspace*{270\p@}}
\makeatother

%----------------------------------------------------------------------------------------
%	HYPERLINKS IN THE DOCUMENTS
%----------------------------------------------------------------------------------------

\usepackage{hyperref}
\hypersetup{hidelinks,backref=true,pagebackref=true,hyperindex=true,colorlinks=false,breaklinks=true,urlcolor= ocre,bookmarks=true,bookmarksopen=false,pdftitle={Title},pdfauthor={Author}}
\usepackage{bookmark}
\bookmarksetup{
open,
numbered,
addtohook={%
\ifnum\bookmarkget{level}=0 % chapter
\bookmarksetup{bold}%
\fi
\ifnum\bookmarkget{level}=-1 % part
\bookmarksetup{color=ocre,bold}%
\fi
}
}

